Exact Verification of ReLU Neural Control Barrier Functions

Control Barrier Functions (CBFs) are a popular approach for safe control of nonlinear systems. In CBF-based control, the desired safety properties of the system are mapped to nonnegativity of a CBF, and the control input is chosen to ensure that the CBF remains nonnegative for all time. Recently, machine learning methods that represent CBFs as neural networks (neural control barrier functions, or NCBFs) have shown great promise due to the universal representability of neural networks. However, verifying that a learned CBF guarantees safety remains a challenging research problem. This paper presents novel exact conditions and algorithms for verifying safety of feedforward NCBFs with ReLU activation functions. The key challenge in doing so is that, due to the piecewise linearity of the ReLU function, the NCBF will be nondifferentiable at certain points, thus invalidating traditional safety verification methods that assume a smooth barrier function. We resolve this issue by leveraging a generalization of Nagumo's theorem for proving invariance of sets with nonsmooth boundaries to derive necessary and sufficient conditions for safety. Based on this condition, we propose an algorithm for safety verification of NCBFs that first decomposes the NCBF into piecewise linear segments and then solves a nonlinear program to verify safety of each segment as well as the intersections of the linear segments. We mitigate the complexity by only considering the boundary of the safe region and by pruning the segments with Interval Bound Propagation (IBP) and linear relaxation. We evaluate our approach through numerical studies with comparison to state-of-the-art SMT-based methods. Our code is available at https://github.com/HongchaoZhang-HZ/exactverif-reluncbf-nips23.

==> backup/DetailsV1.tex <==
\section{Verification Algorithm}
\label{sec:verification}
The preceding proposition motivates our overall approach, which is summarized in the following steps:
\begin{enumerate}
    \item[\textbf{Step 1}] We conduct coarser-to-finer search by gridifying the state space into hyper-cubes and use linear relaxation based perturbation analysis (LiRPA) to identify grid squares that intersect the boundary $\{x: b(x) = 0\}$.  %identify those with $b(x)=0$ with linear relaxation based perturbation analysis (LiRPA). 
    \item[\textbf{Step 2}] We  enumerate all possible activation sets within each hyper-cube using Interval Bound Propagation (IBP). We then identify the activation sets and intersections that satisfy $b(x)=0$ using linear programming. 
    \item[\textbf{Step 3}] For each $\mathbf{S}$, we verify that (\ref{eq:neural-containment}) holds (correctness) and verify that the conditions (\ref{eq:safety-ineq-1}) and (\ref{eq:safety-ineq-2}) are satisfied (feasibility).
    % For each $i,j$ and $\{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\} \subseteq \mathcal{S}_{ij}$ with $\overline{\mathcal{X}}(\mathbf{S}_{1}) \cap \cdots \cap \overline{\mathcal{X}}(\mathbf{S}_{r}) \neq \emptyset$, verify that the conditions (\ref{eq:safety-ineq-1}) and (\ref{eq:safety-ineq-2}) are satisfied.
\end{enumerate}

In what follows, we describe each step in detail. We first present an approach and algorithm for enumerating the activation sets at the boundary. We then map the problem of verifying safety of each activation set, as well as safety verification of intersections of activation sets, to nonlinear programs. Finally, we give a proof of correctness for our overall approach. 
% We next present detailed method of enumeration and verification in Section \ref{subsec:enumerating} and \ref{subsec:verification}, respectively. 

\subsection{Enumeration}
\label{subsec:enumerating}

% We conduct coarser-to-finer search by gridifying the state space in to hyper-cubes and identify those with $b(x)=0$ with linear relaxation based perturbation analysis (LiRPA). 
% We next enumerate all possible activation sets within each hyper-cube using Interval Bound Propagation (IBP). We then identify the activation sets and intersections that satisfy $b(x)=0$ using linear programming. 

% \begin{problem}
% \label{prob:search}
% Given a neural network function $b: \mathcal{X} \rightarrow \mathbb{R}$ with ReLU activation function, find all linear piece with corresponding activated set $\mathbf{S}$ and all non-differentiable intersections $\mathbf{V}$. 
% \end{problem}

We next present the approach to enumerate activation sets of a given ReLU NCBF that intersect the safety boundary, i.e. $b(x)=0$. Intuitively, one can take coarser-to-finer search for activation set that intersect with the safety boundary. Specifically, we first identify regions that contain $b(x)=0$, then enumerate all possible activation sets within the region and finally identify the sets that intersect the safety boundaries. The advantage of this approach that it allows the search algorithm to quickly eliminate large areas of the search space that do not intersect the boundary $b(x)=0$. The details of our approach to enumerating the activated sets are stated as follows. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/illustrate_search.jpg}
    \caption{Illustration of proposed coarser-to-finer searching method. Hyper-cubes that intersect the safety boundaries are marked in red in gridified state space. With all possible activation sets are listed, we can then identify exact activation set and intersections. }
    \label{fig:my_label}
\end{figure}

We first gridify the given state space $\mathcal{X}$ into hyper-cubes. Then we compute lower and upper bounds $b_l$, $b_u$ of each hyper-cube with linear relaxation based perturbation analysis (LiRPA), i.e., auto LiRPA \cite{xu2020automatic} and pick cubes that have bounds with different signs. We denote the hyper-cubes as $B:=\{x \mid b_l\leq x \leq b_u\}$, for some $b_l$, $b_u$ and the set of ones as $\mathcal{B}:=\{B\mid b(x)=0, \text{for some }x\in B \}$. As is shown in Fig \ref{fig:my_label}, squares $B$ are marked in red. 

Next, we enumerate all possible activation sets in each $B$. We utilize Interval Bound Propagation (IBP) to list unstable neurons that can switch sign within the given region $B$. We collect all possible combinations of activation set $\boldsymbol{S}$ as a set of possible activation sets $\Tilde{\mathcal{S}}$. Note that $\boldsymbol{S} \in \Tilde{\mathcal{S}}$ is possible but may not intersect with $b(x)=0$. 

To identify the exact activation sets that intersect the safety boundaries, we prune the set $\Tilde{\mathcal{S}}$ by attempting to find a solution to the set of linear inequalities
\begin{equation}
\begin{split}
    \label{eq:linearfeasible}
     \overline{W}(\mathbf{S})^{T}x + \overline{r}(\mathbf{S}) = 0 \\
     \overline{W}_{ij}(\mathbf{S})^{T}x + \overline{r}_{ij}(\mathbf{S}) \geq 0 \ \forall (i,j) \in \mathbf{S} \\
     \overline{W}_{ij}(\mathbf{S})^{T}x + \overline{r}_{ij}(\mathbf{S}) \leq 0 \ \forall (i,j) \notin \mathbf{S}
\end{split}
\end{equation}
We denote the pruned set as $\mathcal{S} \subseteq \Tilde{\mathcal{S}}$, as shown in \ref{fig:my_label}. In addition, we search for intersections $\mathcal{V}:=\{\chi(\mathbf{S}_i) \cap B \cap b(x)=0, \ \forall \mathbf{S}_i\in \mathcal{S} \}$ for each hyper-cube $B$. Finally, we output $\mathcal{S}$ and $\mathcal{V}$. 

\subsection{Verifying Safety of Each Activation Set}
\label{subsec:verification}
% \begin{problem}
% \label{prob:verify}
% Given a nonlinear continuous-time system (\ref{eq:dyn}), a set of linear function $b: \mathcal{X} \rightarrow \mathbb{R}$, a set of admissible control inputs $\mathcal{U}$, a safe set $\mathcal{C}$ and an initial state $x_{0} \in \mathcal{D} \subseteq \mathcal{C}$, verify whether $b$ is feasible and correct.
% \end{problem}

The following result gives an equivalent condition for verifying that there is no safety counterexample in the interior of $\overline{\mathcal{X}}(\mathbf{S})$ for a given activation set $\mathbf{S}$.

\begin{lemma}
\label{lemma:single-activation-set-condition}
There is no safety counterexample in the set $\overline{\mathcal{X}}(\mathbf{S}) \setminus \bigcup_{\mathbf{S}^{\prime} \neq \mathbf{S}}{\overline{\mathcal{X}}(\mathbf{S})}$ if and only if:
\begin{enumerate}
    \item There do not exist $x \in \mathcal{X}$ and $y \in \mathbb{R}^{p+1}$ satisfying (a) $x \in \mbox{int}(\overline{\mathcal{X}}(\mathbf{S}))$, (b) $b(x) = 0$, (c) $y \geq 0$, (d) $y^{T}\left(\begin{array}{c} -\overline{W}(\mathbf{S})^{T}g(x) \\ A \end{array} \right) = 0$, and (e) $y^{T}\left(\begin{array}{c}\overline{W}(\mathbf{S})^{T}f(x) \\ c\end{array}\right) < 0$.
    \item There does not exist $x \in \mathcal{X}$ with $b(x) = 0$, $x \in \mbox{int}(\overline{\mathcal{X}}(\mathbf{S}))$, and $h(x) < 0$.
\end{enumerate}
\end{lemma}
%\textcolor{blue}{proof omitted}

The proof can be found in the supplementary material. Conditions 1 and 2 of Lemma \ref{lemma:single-activation-set-condition} can be verified by solving  nonlinear programs.  
%\begin{equation}
%\label{eq:single-set-nonlinear-prog}
%\begin{array}{ll} 
%\min_{x,y} & y^{T}\left(
%\begin{array}{c}
%\overline{W}(\mathbf{S})^{T}f(x) \\
%c
%\end{array}
%\right) \\
%\mbox{s.t.} & y^{T}\left(
%\begin{array}{c}
%-\overline{W}(\mathbf{S})^{T}g(x) \\
%A
%\end{array}
%\right) = 0 \\
%& y \geq 0 \\
%& \overline{W}(S)^{T}x + \overline{r}(\mathbf{S}) = 0 %\\
%& \overline{W}_{ij}(\mathbf{S})^{T}x + %\overline{r}_{ij}(\mathbf{S}) > 0 \ \forall (i,j) \in %\mathbf{S} \\
%& \overline{W}_{ij}(\mathbf{S})^{T}x + \overline{r}_{ij}(\mathbf{S}) < 0 \ \forall (i,j) \notin S
%\end{array}
%\end{equation}
%and checking whether the optimal value is nonnegative (safe) or negative (unsafe).

The following corollary describes the special case where there are no constraints on the control, i.e., $\mathcal{U} = \mathbb{R}^{m}$.

\begin{corollary}
    \label{corollary:single-set-unbounded}
    If $\mathcal{U} = \mathbb{R}^{m}$, then there is no safety counterexample in the set $\overline{\mathcal{X}}(S) \setminus \bigcup_{\mathbf{S}^{\prime} \neq \mathbf{S}}{\overline{\mathcal{X}}(\mathbf{S}^{\prime})}$ if and only if (1) there does not exist $x \in \mathcal{X}$ satisfying $x \in \mbox{int}(\overline{\mathcal{X}}(\mathbf{S}))$, $b(x) = 0$, $\overline{W}(\mathbf{S})^{T}g(x) = 0$, and $\overline{W}(\mathbf{S})^{T}f(x) < 0$ and (2)  there does not exist $x \in \mathcal{X}$ with $b(x) = 0$, $x \in \mbox{int}(\overline{\mathcal{X}}(\mathbf{S}))$, and $h(x) < 0$.
\end{corollary}

Under the conditions of Corollary \ref{corollary:single-set-unbounded}, the complexity of the verification problem can be reduced. 
%Under the conditions of Corollary \ref{corollary:single-set-unbounded}, the nonlinear program (\ref{eq:single-set-nonlinear-prog}) reduces to 
%\begin{equation}
%\label{eq:single-set-nonlinear-prog-special-case}
%\begin{array}{ll} 
%\min_{x} & \overline{W}(\mathbf{S})^{T}f(x) \\
%\mbox{s.t.} 
%& \overline{W}(\mathbf{S})^{T}g(x) = 0 \\
%& \overline{W}(S)^{T}x + \overline{r}(\mathbf{S}) = 0 %\\
%& \overline{W}_{ij}(\mathbf{S})^{T}x + \overline{r}_{ij}(\mathbf{S}) > 0 \ \forall (i,j) \in \mathbf{S} \\
%& \overline{W}_{ij}(\mathbf{S})^{T}x + \overline{r}_{ij}(\mathbf{S}) < 0 \ \forall (i,j) \notin S
%\end{array}
%\end{equation}
If $g(x)$ is a constant matrix $G$, then safety is automatically guaranteed if $\overline{W}(\mathbf{S})^{T}G \neq 0$. If $f(x)$ is linear in $x$ as well, then verification can be performed via a linear program. %When $x$ is nonlinear but $f(x)$ is bounded within a particular region for all $x \in \overline{\mathcal{X}}(\mathbf{S})$ with $b(x) = 0$, Eq. (\ref{eq:single-set-nonlinear-prog-special-case}) can be relaxed 

Turning to Condition 2, it suffices to solve the nonlinear program
\begin{equation}
\label{eq:containment-verification}
\begin{array}{ll}
\mbox{minimize} & h(x) \\
\mbox{s.t.} & \overline{W}_{ij}(\mathbf{S})^{T}x + \overline{r}_{ij}(\mathbf{S}) \geq 0 \ \forall (i,j) \in \mathbf{S} \\
& \overline{W}_{ij}(\mathbf{S})^{T}x + \overline{r}_{ij}(\mathbf{S}) \leq 0 \ \forall (i,j) \notin \mathbf{S} \\
& \overline{W}(\mathbf{S})^{T}x + \overline{r}(\mathbf{S}) = 0
\end{array}
\end{equation}
and check whether the optimal value is nonnegative (unsafe) or negative (safe).

\subsection{Verification of Activation Set Boundaries}
\label{subsec:verification-boundary}
We now describe an approach for verifying safety of intersections between activation sets.

\begin{lemma}
\label{lemma:multi-activation-set-condition}
Suppose that the sets $\mathbf{S}_{1},\ldots,\mathbf{S}_{r}$ satisfy condition (ii) of Lemma \ref{lemma:single-activation-set-condition}. There is no safety counterexample in the set $$\overline{\mathcal{X}}(\mathbf{S}_{1}) \cap \cdots \cap \overline{\mathcal{X}}(\mathbf{S}_{r}) \setminus \bigcup_{S^{\prime} \notin \{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\}}{\overline{\mathcal{X}}(\mathbf{S}^{\prime})}$$ if and only if there do not exist $x \in \mathcal{X}$ and $y_{1},\ldots,y_{r} \in \mathbb{R}^{T + p+1}$, where $T = |\mathbf{T}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r})|$, satisfying (a) $x \in \mbox{int}(\overline{\mathcal{X}}(\mathbf{S}_{1})) \cap \cdots \cap \mbox{int}(\overline{\mathcal{X}}(\mathbf{S}_{r}))$, (b) $b(x) = 0$, (c) $y_{l} \geq 0$ for all $l=1,\ldots,r$, (d) for all $l=1,\ldots,r$  , $y_{l}^{T}\Theta_{l}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r}(x)) = 0$, where $\Theta_{l}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r},x)$ is a $(T+p+1) \times m$ matrix given by
\begin{equation}
    \Theta_{l}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r},x) \triangleq \left(
    \begin{array}{c}
    -W_{ij}(\mathbf{S}_{l})^{T}g(x) : (i,j) \in \mathbf{T}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r}) \cap \mathbf{S}_{l} \\
    W_{ij}(\mathbf{S}_{l})^{T}g(x) : (i,j) \in \mathbf{T}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r}) \setminus \mathbf{S}_{l} \\
    -W_{ij}(\mathbf{S}_{l}^{T}g(x) \\
    A
    \end{array}
    \right)
\end{equation}
%\begin{equation}
%\label{eq:multiple-set-1}
%y_{l}^{T}\underbrace{\left(
%\begin{array}{c}
%-W_{i_{1}j_{1}}(\mathbf{S}_{l})^{T}g(x) \\
%\vdots \\
%-W_{i_{T}j_{T}}(\mathbf{S}_{l})^{T}g(x) \\
%-W(\mathbf{S}_{l})^T{}g(x) \\
%A
%\end{array}
%\right)}_{\triangleq \Theta_{l}%(\mathbf{S}_{1},\ldots,\mathbf{S}_{r},x)} = 0,
%\end{equation}
and (e) for all $l=1,\ldots,r$, $y_{l}^{T}\Lambda_{l}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r},x) < 0$, where $\Lambda_{l}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r},x) \in \mathbb{R}^{T+p+1}$ is given by
\begin{equation}
    \Lambda_{l}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r},x) \triangleq \left(
    \begin{array}{c}
    \overline{W}_{ij}(\mathbf{S}_{l})^{T}f(x) : (i,j) \in \mathbf{T}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r}) \cap \mathbf{S}_{l} \\
    -\overline{W}_{ij}(\mathbf{S}_{l})^{T}f(x) : (i,j) \in \mathbf{T}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r}) \setminus \mathbf{S}_{l} \\
    \overline{W}(\mathbf{S}_{l})^{T}f(x) \\
    c
    \end{array}
    \right)
    \end{equation}
%\end{equation}
%\begin{equation}
%\label{eq:multiple-set-2}
%y_{l}^{T}\underbrace{\left(
%\begin{array}{c}
%\overline{W}_{i_{1}j_{1}}(\mathbf{S}_{l})^{T}f(x) \\
%\vdots \\
%\overline{W}_{i_{T}j_{T}}(\mathbf{S}_{l})^{T}f(x) \\
%\overline{W}(\mathbf{S}_{l})^{T}f(x) \\
%c
%\end{array}
%\right)}_{\triangleq \Lambda_{l}%(\mathbf{S}_{1},\ldots,\mathbf{S}_{r},x)} < 0
%\end{equation}
%\end{enumerate}
\end{lemma}

The proof can be found in the supplementary material. The verification problem can then be mapped to solving the nonlinear program
\begin{equation}
\label{eq:multiple-set-nonlinear-program}
\begin{array}{ll}
\mbox{min}_{x,y_{1},\ldots,y_{r}} & \max_{l=1,\ldots,r}{\left\{y_{l}^{T}\left(\begin{array}{c}
\overline{W}_{i_{1}j_{1}}(\mathbf{S}_{l})^{T}f(x) \\
\vdots \\
\overline{W}_{i_{T}j_{T}}(\mathbf{S}_{l})^{T}f(x) \\
c
\end{array}
\right)\right\}} \\
\mbox{s.t.} & \overline{W}_{ij}(\mathbf{S}_{1})^{T}x + \overline{r}_{ij}(\mathbf{S}_1) < 0 \ \forall (i,j) \notin S_{1} \cup \cdots \cup S_{r} \\
& \overline{W}_{ij}(\mathbf{S}_{1})^{T}x + \overline{r}_{ij}(\mathbf{S}_{1}) > 0 \ \forall (i,j) \in S_{1} \cap \cdots \cap S_{r} \\
& \overline{W}_{ij}(\mathbf{S}_{1})^{T}x + \overline{r}_{ij}(\mathbf{S}_{1}) = 0 \ \forall (i,j) \in \mathbf{T}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r}) \\
& y_{l}^{T}\Theta_{l}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r}(x)) = 0 \ \forall l=1,\ldots,r \\
& y_{l} \geq 0 \ \forall l=1,\ldots,r
\end{array}
\end{equation}
and checking whether the optimal value is nonnegative (safe) or negative (unsafe). 
Note that, if $g(x)$ is constant, then the constraints of (\ref{eq:multiple-set-nonlinear-program}) are linear, and if $f(x)$ is linear then (\ref{eq:multiple-set-nonlinear-program}) reduces to solving a system of linear and bilinear inequalities. Furthermore, if $f(x)$ can be bounded over $x \in \overline{\mathcal{X}}(\mathbf{S}_{1}) \cap \cdots \cap \overline{\mathcal{X}}(\mathbf{S}_{r})$ and $b(x) = 0$, then this bound can be used to derive a linear relaxation to the objective function of (\ref{eq:multiple-set-nonlinear-program}), thus relaxing the nonlinear program to a linear program. 

The complexity of this approach can also be reduced by utilizing sufficient conditions for safety that are easier to check. For instance, if there exists $u \in \mathcal{U}$ such that $\overline{W}(\mathbf{S})^{T}(f(x) + g(x)u) \geq 0$ for all $\mathbf{S} \in \mathbf{S}(x)$, then the criteria of Lemma \ref{lemma:multi-activation-set-condition} are satisfied. In particular, if $\overline{W}(\mathbf{S})^{T}f(x) \geq 0$ for all $\mathbf{S} \in \mathbf{S}(x)$, then the conditions are satisfied with $u = 0$. 

%\textcolor{blue}{revise notations*} Besides, we present sufficient conditions for verification of activation set boundaries. In NBF verification, one can check if $\min_x{\overline{W}(\mathbf{S}_i)f(x)}\geq0$, $\forall x\in \cap_i\mathbf{S}_{i}$ for some all $\mathbf{S}_{i}\in \boldsymbol{V}$. In NCBF verification without constraints on control input, one can check if the sign of $\overline{W}(\mathbf{S}_i)g(x)$ are consistent for $\boldsymbol{S}_i \in \boldsymbol{V}$. Note that these sufficient conditions decrease computational complexity in practical. However, if the sufficient conditions do not hold, it does not necessary means the verification fails. One can can refer to \eqref{multiple-set-nonlinear-program} for necessary and sufficient verification. 

% \subsection{Proof of Correctness}
% \label{subsec:overall-proof}
The following result summarizes the correctness of our overall approach.

\begin{theorem}
\label{theorem:overall-verification-proof}
Suppose that the conditions of Lemma \ref{lemma:single-activation-set-condition} are satisfied for each $\mathbf{S} \in \mathcal{S}$ and the conditions of Lemma \ref{lemma:multi-activation-set-condition} are satisfied for each $(\mathbf{S}_{1},\ldots,\mathbf{S}_{r}) \in \mathcal{V}$. Then the NCBF $b$ is consistent and feasible. 
%For each $i=1,\ldots,M$, let $\mathcal{Z}_{i}$ denote the set of points where a line from $x_{0}$ to $U_{i}$ intersects $\partial\mathcal{C}$. For each $x_{ij} \in \mathcal{Z}_{i}$, let $(\mathcal{S}_{ij}, \mathcal{V}_{ij})$ denote the activation sets and intersections when $x_{ij}$ is given as input. Suppose that the following conditions hold: (a) For all $\mathbf{S} \in \mathcal{S}_{ij}$, the value of the nonlinear program (\ref{eq:single-set-nonlinear-prog}) is nonnegative; (b) For all $\mathbf{S} \in \mathcal{S}_{ij}$, the value of the nonlinear program $\min{\{h(x) : x \in \overline{\mathcal{X}}_{0}(\mathbf{S})\}}$ is negative; and (c) For all $\{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\} \in \mathcal{V}_{ij}$, the value of the nonlinear program (\ref{eq:multiple-set-nonlinear-program}) is nonnegative. Then any control policy that is consistent with $b$ is safe.
\end{theorem}

\begin{proof}
    Suppose that $x$ is a safety counterexample for the NCBF $b$ with $b(x) = 0$. If $x \in \mbox{int}\overline{\mathcal{X}}(\mathbf{S})$ for some $\mathbf{S}$, then we have that $\mathbf{S} \in \mathcal{S}$ and hence a contradiction with Lemma \ref{lemma:single-activation-set-condition}. If $x \in \overline{\mathcal{X}}(\mathbf{S}_{1}) \cap \cdots \overline{\mathcal{X}}(\mathbf{S}_{r})$ for some $\mathbf{S}_{1},\ldots,\mathbf{S}_{r}$, then there is a contradiction with Lemma \ref{lemma:multi-activation-set-condition}. 
\end{proof}

%Theorem \ref{theorem:overall-verification-proof} implies that, if passing the verification, then any control policy consistent with barrier function $b$ will be safe. 

==> backup/ExperimentV1.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we evaluate our proposed method to verify neural control barrier functions on three systems. We first consider the Darboux system~\cite{zeng2016darboux}, a nonlinear open-loop polynomial system that has been widely used for safety verification. We then evaluate our approach on an obstacle avoidance scenario~\cite{barry2012safety}. We finally evaluate our approach on a spacecraft rendezvous problem from~\cite{jewison2016spacecraft}. The experiments run on a 64-bit Windows PC with Intel(R) Core(TM) i7-12700 processor, 32GB RAM and NVIDIA GeForce RTX 3080 GPU. 

\subsection{Darboux}
We first show verification of a neural barrier function for Darboux system whose dynamic is defined as follow. 
\begin{equation}
    \left[\begin{array}{c}
    \dot{x}_1 \\
    \dot{x_2}
    \end{array}\right]=\left[\begin{array}{c}
    x_2+2 x_1 x_2 \\
    -x_1+2 x_1^2-x_2^2
    \end{array}\right].
\end{equation}
We define state space, initial region, and unsafe region as $\mathcal{X}:\left\{\mathbf{x} \in \mathbb{R}^2: x\in[-2,2]\times[-2,2] \right\}$, $\mathcal{X}_I:\left\{\mathbf{x} \in \mathbb{R}^2: 0 \leq x_1 \leq 1,1 \leq x_2 \leq 2\right\}$ and $\mathbf{x}_{U}:\left\{\mathbf{x} \in \mathbb{R}^2: x_1+x_2^2 \leq 0\right\}$ respectively. 

We first show an example of correctness verification. We construct a neural barrier function with one hidden layer consisting of 20 neurons followed with a ReLU activation function. We  trained two NBFs that (a) terminated after $3$ epochs and (b) completed training. As shown in Fig. \ref{fig:Darboux_failure}, the NBF with unfinished training has a boundary that intersects the unsafe region, hence, this barrier function is used to test whether our approach can correctly identify that an NBF does not ensure safety. The fully-trained NBF  has a boundary shown in Fig. \ref{fig:Darboux_succ} that  separates the safe and unsafe regions. 

We next verify the NBFs with our proposed method and compared our total run time with state-of-the-art SMT-based verification, dReal and Z3. We first verified a network with 1 ReLU hidden layer and 20 neurons in each hidden layer. The NBF passed all components of the verification after $0.43s$ seconds(s) in total. The enumerating procedure takes $0.39s$ to find $13$ activation set and intersections. The sufficient condition verification takes $0.04s$. The SMT-based verification dReal verified the NBF in $0.36s$ in total. The SMT-based verification Microsoft Z3 cannot finish within an hour when verifying the NBF. 
We first verified a network with 2 ReLU hidden layer and 10 neurons in each hidden layer. The NBF passed all components of the verification after $0.47s$ seconds(s) in total. The enumerate set procedure takes $0.42s$ to find $4$ activation set and intersections. The sufficient condition verification takes $0.05s$. The SMT-based verification takes $7.70s$ with dReal and $15.81$ with Microsoft Z3. 

\begin{figure}[!htbp]
\centering
\begin{subfigure}{.24\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{figs/Darboux_1_5_incorrect.png}
  \subcaption{}
  \label{fig:Darboux_failure}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/Darboux_1_20_correct.png}
%   \caption{Joint FDI and Spoofing Attack: INS2 estimation}
  \subcaption{}
  \label{fig:Darboux_succ}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_1_10_fail.png}
%   \caption{Joint FDI and Spoofing Attack: INS2 estimation}
  \subcaption{}
  \label{fig:obs_fail}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_succ.png}
%   2-16
  \subcaption{}
  \label{fig:obs_succ}
\end{subfigure}%
\caption{Visualization of neural barrier functions. (a) Barrier function training with insufficient data results in a boundary (black, blue, and yellow lines) that intersects with the unsafe region (red area). Our verification algorithm identifies this safety violation. (b) Training with sufficient data results in a boundary that avoids the unsafe region.}
\label{fig:DarbouxRes}
\end{figure}

\subsection{Obstacle Avoidance}
We next evaluate that our proposed method on a controlled system~\cite{barry2012safety}. We consider an Unmanned aerial vehicle (UAVs) flying  through a forest avoiding collision with tree trunks. We model the system as a  Dubins-style \cite{dubins1957curves} aircraft model. The system state  consists of 2-D position and aircraft yaw rate $x:=[x_1, x_2, \psi]^T$. We let $u$ denote the control input to manipulate yaw rate and define the dynamics as
\begin{equation}
    \left[\begin{array}{c}
    \dot{x}_1 \\
    \dot{x}_2 \\
    \dot{\psi}
    \end{array}\right]=\left[\begin{array}{c}
    v \sin \psi \\
    v \cos \psi \\
    0
\end{array}\right]
+ \left[\begin{array}{c}
    0 \\
    0 \\
    u
\end{array}\right]. 
\end{equation}
We define the state space, initial region and unsafe region as $\mathcal{X}$, $\mathcal{X}_I$ and $\mathcal{X}_U$, respectively as 
\begin{equation}
    \begin{aligned}
    \mathcal{X}:&\left\{\mathbf{x} \in \mathbb{R}^3:x_1,x_2,\psi\in [-2,2]\times[-2,2]\times[-2,2] \right\} \\
    \mathcal{X}_I:&\left\{\mathbf{x} \in \mathbb{R}^3:-0.1 \leq x_1 \leq 0.1,-2 \leq x_2 \leq-1.8, \ -\pi/6<\psi<\pi / 6 \right\} \\
    \mathcal{X}_U:&\left\{\mathbf{x} \in \mathbb{R}^3: x_1^2+x_2^2 \leq 0.04\right\}
\end{aligned}
\end{equation}
We obtain the trained NCBF by CEGIS framework in \cite{zhao2020synthesizing} with $v$ assumed to be $1$ and the control law $u$ designed as
$ u=-\sin \psi+3 \cdot \frac{x_1 \cdot \sin \psi+x_2 \cdot \cos \psi}{0.5+x_1^2+x_2^2}$. 

We next verify the NCBFs with our proposed method. We first verified a network with 1 ReLU hidden layer and 50 neurons in each hidden layer. The NCBF passed all components of the verification after $13.86s$ in total. The enumerating procedure takes $12.81s$ to find $966$ activation set and intersections. The sufficient condition verification takes $1.06s$. 
We then verified a network with 2 ReLU hidden layer and 32 neurons in each hidden layer. The NBF passed all components of the verification after $273.37s$ seconds(s) in total. The enumerate set procedure takes $218.86s$ to find $1317$ activation set and intersections. The sufficient condition verification takes $54.51s$. 

\subsection{Spacecraft Rendezvous}
The state of the chaser is expressed relative to the target using linearized Clohessy–Wiltshire–Hill equations, with state $x=[p_x, p_y, p_z, v_x, v_y, v_z]^T$, control input $u=[u_x, u_y, u_z]^T$ and dynamics defined as follows. 
\begin{equation}
    \left[\begin{array}{c}
    \dot{p}_x \\
    \dot{p}_y \\
    \dot{p}_z \\
    \dot{v}_x \\
    \dot{v}_y \\
    \dot{v}_z
    \end{array}\right]=
    \left[\begin{array}{c c c c c c}
    1 &0 &0 &0 &0 &0 \\
    0 &1 &0 &0 &0 &0 \\
    0 &0 &1 &0 &0 &0 \\
    3n^2 &0 &0 &0 &2n &0 \\
    0 &0 &0 &-2n &0 &0 \\
    0 &0 &-n^2 &0 &0 &0 
    \end{array}\right]
    \left[\begin{array}{c}
    p_x \\
    p_y \\
    p_z \\
    v_x \\
    v_y \\
    v_z
    \end{array}\right]
+ \left[\begin{array}{c c c}
    0 &0 &0 \\
    0 &0 &0 \\
    0 &0 &0 \\
    1 &0 &0 \\
    0 &1 &0 \\
    0 &0 &1
\end{array}\right]
\left[\begin{array}{c}
    u_x \\
    u_y \\
    u_z 
    \end{array}\right]. 
\end{equation}
We define the state space, initial region and unsafe region as $\mathcal{X}$, $\mathcal{X}_I$ and $\mathcal{X}_U$, respectively as 
\begin{equation}
    \begin{aligned}
    \mathcal{X}:&\left\{\mathbf{x} \in \mathbb{R}^3: p, v, \in [-1.5,1.5]\times[-1.5,1.5]\right\} \\
    \mathcal{X}_U:&\left\{ 0.25 \leq r \leq 1.5\text{, where } r=\sqrt{p_x^2+ p_y^2+ p_z^2} \right\}
\end{aligned}
\end{equation}

We obtain the trained NCBF with neural CLBF training in~\cite{dawson2023safe} with a nominal model predictive controller. We next verify the NCBFs with our proposed method. We first verified a NCBF who has 2 ReLU hidden layers with 8 neurons in each hidden layer and 1 hidden layer with linear activation function. The NCBF passed all components of the verification after $47.45s$ in total. The enumerating procedure takes $47.45s$ to find $273$ activation set and intersections. The sufficient condition verification takes $0.08s$. In this experiment, we observe the increasing dimension can highly increase time consumed for gridifying the state space and LiRPA. Instead, we enumerate $2^8$ activation sets and verified the NCBF. 

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Models & n & NN Strucutre  & $t_e$ & $t_v$  & $T$ & $T_{dReal}$ & $T_{Z3}$ \\ \hline
Darboux & 2 & 2-20-$\sigma$-1         & 0.39 & 0.04 & 0.43    & 0.36 & Null \\
Darboux & 2 & 2-32-$\sigma$-1         & 0.23 & 0.03 & 0.27    & 1.27 & Null \\
Darboux & 2 & 2-64-$\sigma$-1         & 1.89 & 0.13 & 2.02    & Null & Null \\
Darboux & 2 & 2-96-$\sigma$-1         & 4.17 & 0.14 & 4.31    & Null & Null \\
Darboux & 2 & 2-128-$\sigma$-1         & 4.77 & 0.03 & 4.90    & Null & Null \\ \hline
Darboux & 2 & 2-10-$\sigma$-10-$\sigma$-1 & 0.42 & 0.05 & 0.47    & 7.70 & 15.81   \\ 
Darboux & 2 & 2-16-$\sigma$-16-$\sigma$-1 & 2.13 & 0.11 & 2.23    & Null & Null   \\ 
Darboux & 2 & 2-32-$\sigma$-32-$\sigma$-1 & 8.35 & 6.28 & 14.64    & Null & Null   \\ 
Darboux & 2 & 2-48-$\sigma$-48-$\sigma$-1 & 13.69 & 0.19 & 13.88    & Null & Null   \\ 
Darboux & 2 & 2-64-$\sigma$-64-$\sigma$-1 & 31.30 & 0.47 & 31.77  & Null & Null   \\ \hline
\end{tabular}
\caption{Comparison of verification mean run-time of NBF and NCBF in seconds over 10 trails. We list number of dimension as $n$, network architecture with $\sigma$ denoting ReLU and run-time of proposed method including time of enumerating $t_e$, time of verification $t_v$ and time in total $T$. We compare the run-time proposed verification of NBF with SMT-based approaches, i.e., dReal $T_{dReal}$ and Z3 $T_{Z3}$.  }
\label{tab:NBFcomparison}
\end{table}

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Models  & n & NN Strucutre        & $t_e$ & $t_v$  & $T$ \\ \hline
Obstacle & 3 & 3-32-$\sigma$-1         & 6.94 & 0.40 & 7.35  \\
Obstacle  & 3 & 3-64-$\sigma$-1         & 19.17 & 1.87 & 21.05  \\
Obstacle  & 3 & 3-96-$\sigma$-1         & 58.96 & 6.26 & 65.22  \\
Obstacle  & 3 & 3-128-$\sigma$-1         & 169.51 & 15.56 & 185.07  \\ 
\hline
Obstacle  & 3 & 3-16-$\sigma$-16-$\sigma$-1 & 18.72 & 2.66 & 21.39 \\ 
Obstacle  & 3 & 3-32-$\sigma$-32-$\sigma$-1 & 218.86 & 54.51 & 273.37 \\
Obstacle  & 3 & 3-48-$\sigma$-48-$\sigma$-1 & 3197.59 & 9.75 & 3207.34 \\ 
Obstacle  & 3 & 3-64-$\sigma$-64-$\sigma$-1 & 11730.28 & 18.22 & 11748.50 \\\hline
\begin{tabular}[c]{@{}c@{}}Spacecraft \\ Rendezvous\end{tabular}  & 6 & 6-8-$\sigma$-8-$\sigma$-8-1 & 78.77 & 10.23  & 89.00  \\ 
\begin{tabular}[c]{@{}c@{}}Spacecraft \\ Rendezvous\end{tabular}  & 6 & 6-16-$\sigma$-16-$\sigma$-16-1 & 1261.604 & 501.062 & 1762.666  \\ \hline
\end{tabular}
\caption{Comparison of verification mean run-time of NBF and NCBF in seconds over 10 trails. We list number of dimension as $n$, network architecture with $\sigma$ denoting ReLU and run-time of proposed method including time of enumerating $t_e$, time of verification $t_v$ and time in total $T$. We compare the run-time proposed verification of NBF with SMT-based approaches, i.e., dReal $T_{dReal}$ and Z3 $T_{Z3}$.  }
\label{tab:comparison}
\end{table}



% 32 counter-example 
% 0.099999237060546878, -1.8141281127929685, 0.51555564880371096
% dbdxf = -1.1600 dbdxg = 0.6226
% Counterexample Found: x0 : [-0.19999999825377018, -0.19999847260187381]
% x1 : [2.6428997918226282e-05, 2.9071897710048909e-05]
% x2 : [-0.72578002929687502, -0.7257785320281982]


\begin{figure}[!htbp]
\centering
\begin{subfigure}{.4\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{figs/LogActSetCmp.png}
  \subcaption{}
  \label{fig:Darboux_failure}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/LogRuntimeComp.png}
%   2-16
  \subcaption{}
  \label{fig:obs_succ}
\end{subfigure}%
\caption{Visualization of neural barrier functions. (a) Barrier function training with insufficient data results in a boundary (black, blue, and yellow lines) that intersects with the unsafe region (red area). Our verification algorithm identifies this safety violation. (b) Training with sufficient data results in a boundary that avoids the unsafe region.}
\label{fig:DarbouxRes}
\end{figure}

==> backup/ExperimentV2.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we evaluate our proposed method to verify neural control barrier functions on three systems, namely Darboux, obstacle avoidance and spacecraft rendezvous. The experiments run on a 64-bit Windows PC with Intel(R) Core(TM) i7-12700 processor, 32GB RAM and NVIDIA GeForce RTX 3080 GPU. 

\subsection{Experiment Setup}
\textbf{Darboux:} We first consider the Darboux system~\cite{zeng2016darboux}, a nonlinear open-loop polynomial system that has been widely used as a benchmark for constructing barrier certificates. The dynamic model is given in \ref{sup:darboux}. We obtain the trained NCBF by following the method proposed in \cite{zhao2020synthesizing}. \textbf{training details}

\textbf{Obstacle Avoidance:} We next evaluate our proposed method on a controlled system~\cite{barry2012safety}. We consider an Unmanned Aerial Vehicles (UAVs) avoiding collision with a tree trunk modeled as an unsafe region. We model the system as a  Dubins-style \cite{dubins1957curves} aircraft model. The system state  consists of 2-D position and aircraft yaw rate $x:=[x_1, x_2, \psi]^T$. We let $u$ denote the control input to manipulate yaw rate and the dynamics defined in \ref{sup:obstacle}. 
We obtain the trained NCBF by training method proposed in \cite{zhao2020synthesizing} with $v$ assumed to be $1$ and the control law $u$ designed as
$ u=-\sin \psi+3 \cdot \frac{x_1 \cdot \sin \psi+x_2 \cdot \cos \psi}{0.5+x_1^2+x_2^2}$. \textbf{training details}

\textbf{Spacecraft Rendezvous:} We finally evaluate our approach on a spacecraft rendezvous problem from~\cite{jewison2016spacecraft}. A station-keeping controller is required to keep the "chaser" satellite with in a certain relative distance to the "target" satellite, modeled as unsafe region. The state of the chaser is expressed relative to the target using linearized Clohessy–Wiltshire–Hill equations, with state $x=[p_x, p_y, p_z, v_x, v_y, v_z]^T$, control input $u=[u_x, u_y, u_z]^T$ and dynamics defined in \ref{sup:Spacecraft}. We obtain the trained NCBF with neural CLBF training in~\cite{dawson2023safe} with a nominal model predictive controller. \textbf{more description} \textbf{training details}

\subsection{Experiment Results}
\begin{figure}[!t]
\centering
\begin{subfigure}{.24\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{figs/Darboux_1_5_incorrect.png}
  \subcaption{}
  \label{fig:Darboux_failure}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/Darboux_1_20_correct.png}
  \subcaption{}
  \label{fig:Darboux_succ}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_1_10_fail.png}
  \subcaption{}
  \label{fig:obs_fail}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_succ.png}
%   2-16
  \subcaption{}
  \label{fig:obs_succ}
\end{subfigure}%
\caption{Visualization of neural barrier functions. We shows $-0.05$, $0$, and $0.05$ level set boundaries in blue, black, and yellow lines, respectively, initial region in green and the unsafe region in red. (a) and (b) compares NBFs for Darboux that fail and pass correctness verification, respectively. (b) Training with sufficient data results in a boundary that avoids the unsafe region. (c) and (d) shows projection of NCBFs for Obstacle Avoidance that fail and pass correctness verification, respectively. }
\label{fig:DarbouxRes}
\end{figure}
\textbf{Correctness Verification: }
We first show examples of correctness verification, namely, NBFs for Darboux and NCBFs for obstacle avoidance. We trained two NBFs. NBF (a) has $1$ hidden layer with $5$ neurons while NBF (b) has $1$ hidden layer with $20$ neurons. NBF (a) terminated after $3$ epochs and (b) completed training. We have NBF (a) failed correctness verification while NBF (b) passed. As shown in Fig. \ref{fig:Darboux_failure}, the NBF (a) with unfinished training has a boundary that intersects the unsafe region while the fully-trained NBF (b) separates the safe and unsafe regions in Fig. \ref{fig:Darboux_succ}. 

We then trained two NCBFs. NCBF (c) has $1$ hidden layer with $10$ neurons while NCBF (d) has $1$ hidden layer with $20$ neurons. NBF (c) terminated after $5$ epochs and (d) completed training. We have NCBF (c) failed correctness verification while NCBF (d) passed. We show the correctness counterexample in 2-D projection with $\phi=-1.5$. As shown in Fig. \ref{fig:obs_fail}, the NCBF (c) has its boundary overlap the unsafe region. Our verification algorithm identifies this safety violation. We show the correctness counterexample in 2-D projection with $\phi=-1.5$. As shown in Fig. \ref{fig:obs_fail}, the NCBF (c) has its boundary overlap the unsafe region. 

These results validate our correctness verification and shows that a NBF/NCBF that fails correctness verification may have the invariant set no longer a subset of the given safe region, hence does not ensure safety. 



\textbf{Feasibility Verification}
We compare the run-time of proposed verification with SMT-based approaches using translator proposed in~\cite{abate2021fossil} and SMT solver dReal~\cite{gao2013dreal} and Z3~\cite{de2008z3}. 

All NBFs for Darboux pass feasibility verification with run-time presented in Table \ref{tab:NBFcomparison}. We can find the proposed method can verify NBFs with more ReLU neurons while SMT-based approaches return nothing within $1$ hour time limit. One of the reason of improvement in performance is that we can reduce complexity by only considering the exact safety boundaries, while SMT-based approaches need to search over a safety critical subset of the state space.  
\begin{table}[!tb]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Models & n & NN Strucutre  & $t_e$ & $t_v$  & $T$ & $T_{dReal}$ & $T_{Z3}$ \\ \hline
 & 2 & 2-20-$\sigma$-1         & 0.39 & 0.04 & 0.43    & 0.36 & Null \\
 & 2 & 2-32-$\sigma$-1         & 0.23 & 0.03 & 0.27    & 1.27 & Null \\
Darboux & 2 & 2-64-$\sigma$-1         & 1.89 & 0.13 & 2.02    & Null & Null \\
 & 2 & 2-96-$\sigma$-1         & 4.17 & 0.14 & 4.31    & Null & Null \\
 & 2 & 2-128-$\sigma$-1         & 4.77 & 0.03 & 4.90    & Null & Null \\ \hline
 & 2 & 2-10-$\sigma$-10-$\sigma$-1 & 0.42 & 0.05 & 0.47    & 7.70 & 15.81   \\ 
 & 2 & 2-16-$\sigma$-16-$\sigma$-1 & 2.13 & 0.11 & 2.23    & Null & Null   \\ 
Darboux & 2 & 2-32-$\sigma$-32-$\sigma$-1 & 8.35 & 6.28 & 14.64    & Null & Null   \\ 
 & 2 & 2-48-$\sigma$-48-$\sigma$-1 & 13.69 & 0.19 & 13.88    & Null & Null   \\ 
 & 2 & 2-64-$\sigma$-64-$\sigma$-1 & 31.30 & 0.47 & 31.77  & Null & Null   \\ \hline
\end{tabular}
\caption{Comparison of verification run-time of NBF in seconds. We list number of dimension as $n$, network architecture with $\sigma$ denoting ReLU and run-time of proposed method including time of enumerating $t_e$, time of verification $t_v$ and time in total $T$. We compare the run-time proposed verification of NBF with SMT-based approaches, i.e., dReal $T_{dReal}$ and Z3 $T_{Z3}$. We use $Null$ to denote the case triggers an hour time-out. }
\label{tab:NBFcomparison}
\end{table}

We then evaluate our proposed verification for NCBFs. We have all NCBFs for obstacle avoidance pass feasiblity verification. The run-time are presented in Table \ref{tab:NCBFcomparison}. We further visualize the trend of the number of activation sets and run-time with respect to the total number of neurons with ReLU activation function in Fig. \ref{fig:trend} in supplementary material. We can find that the logarithm activation sets size grow steadily with the size of neural network increasing, while the number of dimension has the commanding influence on the size. The logarithm run-time determined by both state dimension and number of ReLU hidden layers. The potential result can be cause by loose activation set estimation. Methods deriving tighter bounds than IBP may mitigate the influence of the ReLU hidden layers. 

We next show that the proposed exact verification do not depend on the quality of nominal controller while existing works are sufficient verification and rely on nominal controllers to conduct neural barrier certificate. Hence, nominal controllers may cause false negative counter examples. We present an example that a valid NCBF may fail barrier certificate with a given controller. The NCBF for obstacle avoidance with one hidden layer and $32$ neurons fails the SMT-based verification using dReal given $ u=-\sin \psi+3 \cdot \frac{x_1 \cdot \sin \psi+x_2 \cdot \cos \psi}{0.5+x_1^2+x_2^2}$. The counter example we have is around the point $(-0.20, 0, -0.73)$. At this point, we have $b(x)=0.0033$, $\frac{\partial b}{\partial x}f(x)=0.0095$, which should be safe using sufficient condition verification. However, the nominal controller makes $\frac{\partial b}{\partial x}(f(x)+g(x)u)=-1.30$ and results in failure of verification. 

\begin{table}[!bp]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Models  & n & NN Strucutre        & $t_e$ & $t_v$  & $T$ \\ \hline
 & 3 & 3-32-$\sigma$-1         & 6.94 & 0.40 & 7.35  \\
Obstacle  & 3 & 3-64-$\sigma$-1         & 19.17 & 1.87 & 21.05  \\
Avoidance  & 3 & 3-96-$\sigma$-1         & 58.96 & 6.26 & 65.22  \\
  & 3 & 3-128-$\sigma$-1         & 169.51 & 15.56 & 185.07  \\ 
\hline
  & 3 & 3-16-$\sigma$-16-$\sigma$-1 & 18.72 & 2.66 & 21.39 \\ 
Obstacle  & 3 & 3-32-$\sigma$-32-$\sigma$-1 & 218.86 & 54.51 & 273.37 \\
Avoidance  & 3 & 3-48-$\sigma$-48-$\sigma$-1 & 3197.59 & 9.75 & 3207.34 \\ 
  & 3 & 3-64-$\sigma$-64-$\sigma$-1 & 11730.28 & 18.22 & 11748.50 \\\hline
Spacecraft  & 6 & 6-8-$\sigma$-8-$\sigma$-8-1 & 78.77 & 10.23  & 89.00  \\ 
Rendezvous  & 6 & 6-16-$\sigma$-16-$\sigma$-16-1 & 1261.60 & 501.06 & 1762.67  \\ 
 & 6 & 6-32-$\sigma$-32-$\sigma$-32-1 & 12108.11 & 1798.08 & 13906.19  \\ \hline
\end{tabular}
\caption{Comparison of verification run-time of NCBF in seconds. }
\label{tab:NCBFcomparison}
\end{table}



% 32 counter-example 
% 0.099999237060546878, -1.8141281127929685, 0.51555564880371096
% dbdxf = -1.1600 dbdxg = 0.6226
% Counterexample Found: x0 : [-0.19999999825377018, -0.19999847260187381]
% x1 : [2.6428997918226282e-05, 2.9071897710048909e-05]
% x2 : [-0.72578002929687502, -0.7257785320281982]
% -(bv+u)
% Out[15]: tensor(-1.3062)
% bv
% Out[16]: tensor(-0.0951)
% u
% Out[17]: tensor(1.4013)


\begin{figure}[!tbp]
\centering
\begin{subfigure}{.4\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{figs/LogActSetCmp.png}
  \subcaption{}
  \label{fig:num_act}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/LogRuntimeComp.png}
%   2-16
  \subcaption{}
  \label{fig:runtime}
\end{subfigure}%
\caption{Comparison of the number of activation sets and run-time with respect to number of neurons in total. (a) shows logarithm of activation set size. (b) shows logarithm of run-time. We denote NBFs for Darboux with 1 and 2 hidden layers as Darboux 1 and Darboux 2, respectively. We denote NCBFs for obstacle avoidance with 1 and 2 hidden layers as obs 1 and obs 2, respectively.}
\label{fig:trend}
\end{figure}

==> backup/ExperimentV3.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we evaluate our proposed method to verify neural control barrier functions on three systems, namely Darboux, obstacle avoidance and spacecraft rendezvous. The experiments run on a 64-bit Windows PC with Intel(R) Core(TM) i7-12700 processor, 32GB RAM and NVIDIA GeForce RTX 3080 GPU. 

\subsection{Experiment Setup}
\textbf{Darboux:} We first consider the Darboux system~\cite{zeng2016darboux}, a nonlinear open-loop polynomial system that has been widely used as a benchmark for constructing barrier certificates. The dynamic model is given in \ref{sup:darboux}. We obtain the trained NCBF by following the method proposed in \cite{zhao2020synthesizing}. \textbf{training details}

\textbf{Obstacle Avoidance:} We next evaluate our proposed method on a controlled system~\cite{barry2012safety}. We consider an Unmanned Aerial Vehicles (UAVs) avoiding collision with a tree trunk modeled as an unsafe region. We model the system as a  Dubins-style \cite{dubins1957curves} aircraft model. The system state  consists of 2-D position and aircraft yaw rate $x:=[x_1, x_2, \psi]^T$. We let $u$ denote the control input to manipulate yaw rate and the dynamics defined in \ref{sup:obstacle}. 
We obtain the trained NCBF by training method proposed in \cite{zhao2020synthesizing} with $v$ assumed to be $1$ and the control law $u$ designed as
$ u=-\sin \psi+3 \cdot \frac{x_1 \cdot \sin \psi+x_2 \cdot \cos \psi}{0.5+x_1^2+x_2^2}$. \textbf{training details}

\textbf{Spacecraft Rendezvous:} We finally evaluate our approach on a spacecraft rendezvous problem from~\cite{jewison2016spacecraft}. A station-keeping controller is required to keep the "chaser" satellite with in a certain relative distance to the "target" satellite, modeled as unsafe region. The state of the chaser is expressed relative to the target using linearized Clohessy–Wiltshire–Hill equations, with state $x=[p_x, p_y, p_z, v_x, v_y, v_z]^T$, control input $u=[u_x, u_y, u_z]^T$ and dynamics defined in \ref{sup:Spacecraft}. We obtain the trained NCBF with neural CBF training in~\cite{dawson2023safe} with a nominal model predictive controller. \textbf{more description} \textbf{training details}

\subsection{Experiment Results}
\begin{figure}[!t]
\centering
\begin{subfigure}{.24\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{figs/Darboux_1_5_incorrect.png}
  \subcaption{}
  \label{fig:Darboux_failure}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/Darboux_1_20_correct.png}
  \subcaption{}
  \label{fig:Darboux_succ}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_1_10_fail.png}
  \subcaption{}
  \label{fig:obs_fail}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_succ.png}
%   2-16
  \subcaption{}
  \label{fig:obs_succ}
\end{subfigure}%
\caption{Visualization of neural barrier functions. We shows $-0.05$, $0$, and $0.05$ level set boundaries in blue, black, and yellow lines, respectively, initial region in green and the unsafe region in red. (a) and (b) compares NBFs for Darboux that fail and pass correctness verification, respectively. (b) Training with sufficient data results in a boundary that avoids the unsafe region. (c) and (d) shows projection of NCBFs for Obstacle Avoidance that fail and pass correctness verification, respectively. }
\label{fig:DarbouxRes}
\end{figure}
\textbf{Correctness Verification: }
We first show examples of correctness verification, namely, NBFs for Darboux and NCBFs for obstacle avoidance. We trained two NBFs. NBF (a) has $1$ hidden layer with $5$ neurons while NBF (b) has $1$ hidden layer with $20$ neurons. NBF (a) terminated after $3$ epochs and (b) completed training. We have NBF (a) failed correctness verification while NBF (b) passed. As shown in Fig. \ref{fig:Darboux_failure}, the NBF (a) with unfinished training has a boundary that intersects the unsafe region while the fully-trained NBF (b) separates the safe and unsafe regions in Fig. \ref{fig:Darboux_succ}. 

We then trained two NCBFs. NCBF (c) has $1$ hidden layer with $10$ neurons while NCBF (d) has $1$ hidden layer with $20$ neurons. NBF (c) terminated after $5$ epochs and (d) completed training. We have NCBF (c) failed correctness verification while NCBF (d) passed. We show the correctness counterexample in 2-D projection with $\phi=-1.5$. As shown in Fig. \ref{fig:obs_fail}, the NCBF (c) has its boundary overlap the unsafe region. Our verification algorithm identifies this safety violation. We show the correctness counterexample in 2-D projection with $\phi=-1.5$. As shown in Fig. \ref{fig:obs_fail}, the NCBF (c) has its boundary overlap the unsafe region. 

These results validate our correctness verification and shows that a NBF/NCBF that fails correctness verification may have the invariant set no longer a subset of the given safe region, hence does not ensure safety. 



\textbf{Feasibility Verification}
We compare the run-time of proposed verification with SMT-based approaches using translator proposed in~\cite{abate2021fossil} and SMT solver dReal~\cite{gao2013dreal} and Z3~\cite{de2008z3}. 

All NBFs for Darboux pass feasibility verification with run-time presented in Table \ref{tab:NBFcomparison}. We can find the proposed method can verify NBFs with more ReLU neurons while SMT-based approaches return nothing within $1$ hour time limit. One of the reason of improvement in performance is that we can reduce complexity by only considering the exact safety boundaries, while SMT-based approaches need to search over a safety critical subset of the state space.  
\begin{table}[!tb]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Models & n & NN Strucutre  & $t_e$ & $t_v$  & $T$ & $T_{dReal}$ & $T_{Z3}$ \\ \hline
 & 2 & 2-20-$\sigma$-1         & 0.39 & 0.04 & 0.43    & 0.36 & Null \\
 & 2 & 2-32-$\sigma$-1         & 0.23 & 0.03 & 0.27    & 1.27 & Null \\
Darboux & 2 & 2-64-$\sigma$-1         & 1.89 & 0.13 & 2.02    & Null & Null \\
 & 2 & 2-96-$\sigma$-1         & 4.17 & 0.14 & 4.31    & Null & Null \\
 & 2 & 2-128-$\sigma$-1         & 4.77 & 0.03 & 4.90    & Null & Null \\ \hline
 & 2 & 2-10-$\sigma$-10-$\sigma$-1 & 0.42 & 0.05 & 0.47    & 7.70 & 15.81   \\ 
 & 2 & 2-16-$\sigma$-16-$\sigma$-1 & 2.13 & 0.11 & 2.23    & Null & Null   \\ 
Darboux & 2 & 2-32-$\sigma$-32-$\sigma$-1 & 8.35 & 6.28 & 14.64    & Null & Null   \\ 
 & 2 & 2-48-$\sigma$-48-$\sigma$-1 & 13.69 & 0.19 & 13.88    & Null & Null   \\ 
 & 2 & 2-64-$\sigma$-64-$\sigma$-1 & 31.30 & 0.47 & 31.77  & Null & Null   \\ \hline
\end{tabular}
\caption{Comparison of verification run-time of NBF in seconds. We list number of dimension as $n$, network architecture with $\sigma$ denoting ReLU and run-time of proposed method including time of enumerating $t_e$, time of verification $t_v$ and time in total $T$. We compare the run-time proposed verification of NBF with SMT-based approaches, i.e., dReal $T_{dReal}$ and Z3 $T_{Z3}$. We use $Null$ to denote the case triggers an hour time-out. }
\label{tab:NBFcomparison}
\end{table}

We then evaluate our proposed verification for NCBFs. We have all NCBFs pass feasiblity verification. The run-time are presented in Table \ref{tab:NCBFcomparison}. We further visualize the trend of the number of activation sets and run-time with respect to the total number of neurons with ReLU activation function in Fig. \ref{fig:trend} in supplementary material. We can find that the logarithm activation sets size grow steadily with the size of neural network increasing, while the number of dimension has the commanding influence on the size. The logarithm run-time determined by both state dimension and number of ReLU hidden layers. The potential result can be cause by loose activation set estimation. Methods deriving tighter bounds than IBP may mitigate the influence of the ReLU hidden layers. 

The proposed exact verification do not depend on the quality of nominal controller while existing works are sufficient verification and rely on nominal controllers to conduct neural barrier certificate. We next show that nominal controllers can create false negative counter examples resulting a valid NCBF failing the verification. The NCBF for obstacle avoidance with one hidden layer and $32$ neurons fails the SMT-based verification using dReal given $ u=-\sin \psi+3 \cdot \frac{x_1 \cdot \sin \psi+x_2 \cdot \cos \psi}{0.5+x_1^2+x_2^2}$. The counter example we have is around the point $(-0.20, 0, -0.73)$. At this point, we have $b(x)=0.0033$, $\frac{\partial b}{\partial x}f(x)=0.0095$, which should be safe using sufficient condition verification. However, the nominal controller makes $\frac{\partial b}{\partial x}(f(x)+g(x)u)=-1.30$ and results in failure of verification. 

\begin{table}[!bp]
\centering
\begin{tabular}{c|c|c|c|c|c}
\hline
Models  & n & NN Strucutre        & $t_e$ & $t_v$  & $T$ \\ \hline
 & 3 & 3-32-$\sigma$-1         & 6.94 & 0.40 & 7.35  \\
Obstacle  & 3 & 3-64-$\sigma$-1         & 19.17 & 1.87 & 21.05  \\
Avoidance  & 3 & 3-96-$\sigma$-1         & 58.96 & 6.26 & 65.22  \\
  & 3 & 3-128-$\sigma$-1         & 169.51 & 15.56 & 185.07  \\ 
\hline
  & 3 & 3-16-$\sigma$-16-$\sigma$-1 & 18.72 & 2.66 & 21.39 \\ 
Obstacle  & 3 & 3-32-$\sigma$-32-$\sigma$-1 & 218.86 & 54.51 & 273.37 \\
Avoidance  & 3 & 3-48-$\sigma$-48-$\sigma$-1 & 3197.59 & 9.75 & 3207.34 \\ 
  & 3 & 3-64-$\sigma$-64-$\sigma$-1 & 11730.28 & 18.22 & 11748.50 \\\hline
Spacecraft  & 6 & 6-8-$\sigma$-8-$\sigma$-8-1 & 78.77 & 10.23  & 89.00  \\ 
Rendezvous  & 6 & 6-16-$\sigma$-16-$\sigma$-16-1 & 1261.60 & 501.06 & 1762.67  \\ 
 & 6 & 6-32-$\sigma$-32-$\sigma$-32-1 & 12108.11 & 1798.08 & 13906.19  \\ \hline
\end{tabular}
\caption{Comparison of verification run-time of NCBF in seconds. }
\label{tab:NCBFcomparison}
\end{table}



% 32 counter-example 
% 0.099999237060546878, -1.8141281127929685, 0.51555564880371096
% dbdxf = -1.1600 dbdxg = 0.6226
% Counterexample Found: x0 : [-0.19999999825377018, -0.19999847260187381]
% x1 : [2.6428997918226282e-05, 2.9071897710048909e-05]
% x2 : [-0.72578002929687502, -0.7257785320281982]
% -(bv+u)
% Out[15]: tensor(-1.3062)
% bv
% Out[16]: tensor(-0.0951)
% u
% Out[17]: tensor(1.4013)


==> backup/ExperimentV4.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we evaluate our proposed method to verify neural control barrier functions on three systems, namely Darboux, obstacle avoidance and spacecraft rendezvous. The experiments run on a 64-bit Windows PC with Intel(R) Core(TM) i7-12700 processor, 32GB RAM and NVIDIA GeForce RTX 3080 GPU. We include training details in the supplement. 

\subsection{Experiment Setup}
\textbf{Darboux:} We first consider the Darboux system~\cite{zeng2016darboux}, a nonlinear open-loop polynomial system that has been widely used as a benchmark for constructing barrier certificates. The dynamic model is given in the supplement. We obtain the trained NCBF by following the method proposed in \cite{zhao2020synthesizing}. 

\textbf{Obstacle Avoidance:} We next evaluate our proposed method on a controlled system~\cite{barry2012safety}. We consider an Unmanned Aerial Vehicles (UAVs) avoiding collision with a tree trunk. We model the system as a  Dubins-style \cite{dubins1957curves} aircraft model. The system state  consists of 2-D position and aircraft yaw rate $x:=[x_1, x_2, \psi]^T$. We let $u$ denote the control input to manipulate yaw rate and the dynamics defined in the supplement. 
We train the NCBF via the method proposed in \cite{zhao2020synthesizing} with $v$ assumed to be $1$ and the control law $u$ designed as
$ u=-\sin \psi+3 \cdot \frac{x_1 \cdot \sin \psi+x_2 \cdot \cos \psi}{0.5+x_1^2+x_2^2}$. 

\textbf{Spacecraft Rendezvous:} We finally evaluate our approach on a spacecraft rendezvous problem from~\cite{jewison2016spacecraft}. A station-keeping controller is required to keep the "chaser" satellite with in a certain relative distance to the "target" satellite. The state of the chaser is expressed relative to the target using linearized Clohessy–Wiltshire–Hill equations, with state $x=[p_x, p_y, p_z, v_x, v_y, v_z]^T$, control input $u=[u_x, u_y, u_z]^T$ and dynamics defined in the supplement. We obtain the trained NCBF via the method proposed in~\cite{dawson2023safe}. 


\begin{figure}[!htp]
\centering
\begin{subfigure}{.24\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{figs/Darboux_1_20_correct.png}
  \subcaption{}
  \label{fig:Darboux_succ}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/Darboux_1_5_incorrect.png}
  \subcaption{}
  \label{fig:Darboux_failure}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_succ.png}
  \subcaption{}
  \label{fig:obs_succ}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_1_10_fail.png}
%   2-16
  \subcaption{}
  \label{fig:obs_fail}
\end{subfigure}%
\caption{Visualization of neural barrier functions. We shows $-0.05$, $0$, and $0.05$ level set boundaries in blue, black, and yellow lines, respectively, initial region in green and the unsafe region in red. (a) and (b) compares NCBFs for Darboux that fail and pass the verification, respectively. (c) and (d) shows projection of NCBFs for Obstacle Avoidance that fail and pass the verification, respectively. }
\label{fig:DarbouxRes}
\end{figure}
\subsection{Experiment Results}
We first verify that $\mathcal{D} \subseteq \mathcal{C}$ with examples of Darboux and obstacle avoidance. We trained two NCBFs. NCBF (a) has $1$ hidden layer with $20$ neurons while NCBF (b) has $1$ hidden layer with $5$ neurons. NCBF (a) completed training and (b) terminated after $3$ epochs. We have NCBF (a) passed the verification while NCBF (b) failed. As shown in Fig. \ref{fig:Darboux_succ}, the fully-trained NCBF (a) separates the safe and unsafe regions while the NCBF (b) with unfinished training has a boundary that intersects the unsafe region in Fig. \ref{fig:Darboux_failure}. 

We then trained two NCBFs. NCBF (c) has $1$ hidden layer with $20$ neurons while NCBF (d) has $1$ hidden layer with $10$ neurons. NCBF (c) completed training and (d) terminated after $5$ epochs. We have NCBF (c) passed the verification while NCBF (d) failed. Our verification algorithm identifies this safety violation. As shown in Fig. \ref{fig:obs_fail}, the 2-D projection with $\psi=-1.5$ of NCBF (d) shows its boundary overlap the unsafe region. These results validate our correctness verification and shows that NCBFs fail the verification can not ensure safety. 

We next verify the positive invariant of $\mathcal{D}$ under dynamics and nominal control policies. All NCBFs for Darboux pass feasibility verification with run-time presented in Table \ref{tab:NBFcomparison}. We compare the run-time of proposed verification with SMT-based approaches using translator proposed in~\cite{abate2021fossil} and SMT solver dReal~\cite{gao2013dreal} and Z3~\cite{de2008z3}. 
We can find the proposed method can verify NCBFs with more ReLU neurons while SMT-based approaches return nothing within $1$ hour time limit. 
\textcolor{blue}{discuss improvement}
% One of the reason of improvement in performance is that we can reduce complexity by only considering the exact safety boundaries, while SMT-based approaches need to search over a safety critical subset of the state space.  
\begin{table}[!tp]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Models & n & NN Strucutre  & $t_e$ & $t_v$  & $T$ & $T_{dReal}$ & $T_{Z3}$ \\ \hline
 & 2 & 2-20-$\sigma$-1         & 0.39 & 0.04 & 0.43    & 0.36 & Null \\
 & 2 & 2-32-$\sigma$-1         & 0.23 & 0.03 & 0.27    & 1.27 & Null \\
Darboux & 2 & 2-64-$\sigma$-1         & 1.89 & 0.13 & 2.02    & Null & Null \\
 & 2 & 2-96-$\sigma$-1         & 4.17 & 0.14 & 4.31    & Null & Null \\
 & 2 & 2-128-$\sigma$-1         & 4.77 & 0.03 & 4.90    & Null & Null \\ \hline
 & 2 & 2-10-$\sigma$-10-$\sigma$-1 & 0.42 & 0.05 & 0.47    & 7.70 & 15.81   \\ 
 & 2 & 2-16-$\sigma$-16-$\sigma$-1 & 2.13 & 0.11 & 2.23    & Null & Null   \\ 
Darboux & 2 & 2-32-$\sigma$-32-$\sigma$-1 & 8.35 & 6.28 & 14.64    & Null & Null   \\ 
 & 2 & 2-48-$\sigma$-48-$\sigma$-1 & 13.69 & 0.19 & 13.88    & Null & Null   \\ 
 & 2 & 2-64-$\sigma$-64-$\sigma$-1 & 31.30 & 0.47 & 31.77  & Null & Null   \\ \hline
\end{tabular}
\caption{Comparison of verification run-time of NCBF in seconds. We list number of dimension as $n$, network architecture with $\sigma$ denoting ReLU and run-time of proposed method including time of enumerating $t_e$, time of verification $t_v$ and time in total $T$. We compare the run-time proposed verification of NCBF with SMT-based approaches, i.e., dReal $T_{dReal}$ and Z3 $T_{Z3}$. We write $Null$ when the program does not terminate in an hour}
\label{tab:NBFcomparison}
\end{table}

We have all NCBFs for obstacle avoidance and spacecraft rendezvous pass the verification. The run-time are presented in Table \ref{tab:NCBFcomparison}. 
We can find that the activation sets size grow steadily with the size of neural network increasing, and the number of dimension has the commanding influence on the size. The run-time is determined by both state dimension and number of ReLU hidden layers. The potential result can be cause by loose activation set estimation. Methods deriving tighter bounds than IBP may mitigate the influence of the ReLU hidden layers. 
% We further visualize the trend of the number of activation sets and run-time with respect to the total number of neurons with ReLU activation function in Fig. \ref{fig:trend} in supplementary material. We can find that the logarithm activation sets size grow steadily with the size of neural network increasing, while the number of dimension has the commanding influence on the size. The logarithm run-time determined by both state dimension and number of ReLU hidden layers. The potential result can be cause by loose activation set estimation. Methods deriving tighter bounds than IBP may mitigate the influence of the ReLU hidden layers. 

The proposed exact verification do not depend on the quality of nominal controller while existing works are sufficient verification and rely on nominal controllers to conduct neural barrier certificate. We next show that nominal controllers can create false negative counter examples resulting a valid NCBF failing the verification. The NCBF for obstacle avoidance with one hidden layer and $32$ neurons fails the SMT-based verification using dReal given $ u=-\sin \psi+3 \cdot \frac{x_1 \cdot \sin \psi+x_2 \cdot \cos \psi}{0.5+x_1^2+x_2^2}$. The counter example we have is around the point $(-0.20, 0, -0.73)$. At this point, we have $b(x)=0.0033$, $\frac{\partial b}{\partial x}f(x)=0.0095$, which should be safe using sufficient condition verification. However, the nominal controller makes $\frac{\partial b}{\partial x}(f(x)+g(x)u)=-1.30$ and results in failure of verification. 

\begin{table}[!bp]
\centering
\begin{tabular}{c|c|c|c|c|c}
\hline
Models  & n & NN Strucutre        & $t_e$ & $t_v$  & $T$ \\ \hline
 & 3 & 3-32-$\sigma$-1         & 6.94 & 0.40 & 7.35  \\
Obstacle  & 3 & 3-64-$\sigma$-1         & 19.17 & 1.87 & 21.05  \\
Avoidance  & 3 & 3-96-$\sigma$-1         & 58.96 & 6.26 & 65.22  \\
  & 3 & 3-128-$\sigma$-1         & 169.51 & 15.56 & 185.07  \\ 
\hline
  & 3 & 3-16-$\sigma$-16-$\sigma$-1 & 18.72 & 2.66 & 21.39 \\ 
Obstacle  & 3 & 3-32-$\sigma$-32-$\sigma$-1 & 218.86 & 54.51 & 273.37 \\
Avoidance  & 3 & 3-48-$\sigma$-48-$\sigma$-1 & 3197.59 & 9.75 & 3207.34 \\ 
  & 3 & 3-64-$\sigma$-64-$\sigma$-1 & 11730.28 & 18.22 & 11748.50 \\\hline
Spacecraft  & 6 & 6-8-$\sigma$-8-$\sigma$-8-1 & 78.77 & 10.23  & 89.00  \\ 
Rendezvous  & 6 & 6-16-$\sigma$-16-$\sigma$-16-1 & 1261.60 & 501.06 & 1762.67  \\ 
 & 6 & 6-32-$\sigma$-32-$\sigma$-32-1 & 12108.11 & 1798.08 & 13906.19  \\ \hline
\end{tabular}
\caption{Comparison of verification run-time of NCBF in seconds. }
\label{tab:NCBFcomparison}
\end{table}



% 32 counter-example 
% 0.099999237060546878, -1.8141281127929685, 0.51555564880371096
% dbdxf = -1.1600 dbdxg = 0.6226
% Counterexample Found: x0 : [-0.19999999825377018, -0.19999847260187381]
% x1 : [2.6428997918226282e-05, 2.9071897710048909e-05]
% x2 : [-0.72578002929687502, -0.7257785320281982]
% -(bv+u)
% Out[15]: tensor(-1.3062)
% bv
% Out[16]: tensor(-0.0951)
% u
% Out[17]: tensor(1.4013)


==> backup/ExperimentV5.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we evaluate our proposed method to verify neural control barrier functions on three systems, namely Darboux, obstacle avoidance and spacecraft rendezvous. The experiments run on a 64-bit Windows PC with Intel(R) Core(TM) i7-12700 processor, 32GB RAM and NVIDIA GeForce RTX 3080 GPU. We include training details in the supplement. 

\subsection{Experiment Setup}
\textbf{Darboux:} We consider the Darboux system~\cite{zeng2016darboux}, a nonlinear open-loop polynomial system that has been widely used as a benchmark for constructing barrier certificates. The dynamic model is given in the supplement. We obtain the trained NCBF by following the method proposed in \cite{zhao2020synthesizing}. 

\textbf{Obstacle Avoidance:} We evaluate our proposed method on a controlled system~\cite{barry2012safety}. We consider an Unmanned Aerial Vehicles (UAVs) avoiding collision with a tree trunk. We model the system as a  Dubins-style \cite{dubins1957curves} aircraft model. The system state  consists of 2-D position and aircraft yaw rate $x:=[x_1, x_2, \psi]^T$. We let $u$ denote the control input to manipulate yaw rate and the dynamics defined in the supplement. 
We train the NCBF via the method proposed in \cite{zhao2020synthesizing} with $v$ assumed to be $1$ and the control law $u$ designed as
$ u=-\sin \psi+3 \cdot \frac{x_1 \cdot \sin \psi+x_2 \cdot \cos \psi}{0.5+x_1^2+x_2^2}$. 

\textbf{Spacecraft Rendezvous:} We evaluate our approach on a spacecraft rendezvous problem from~\cite{jewison2016spacecraft}. A station-keeping controller is required to keep the "chaser" satellite with in a certain relative distance to the "target" satellite. The state of the chaser is expressed relative to the target using linearized Clohessy–Wiltshire–Hill equations, with state $x=[p_x, p_y, p_z, v_x, v_y, v_z]^T$, control input $u=[u_x, u_y, u_z]^T$ and dynamics defined in the supplement. We obtain the trained NCBF via the method proposed in~\cite{dawson2023safe}. 


\begin{figure}[!tp]
\centering
\begin{subfigure}{.24\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{figs/Darboux_1_20_correct.png}
  \subcaption{}
  \label{fig:Darboux_succ}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/Darboux_1_5_incorrect.png}
  \subcaption{}
  \label{fig:Darboux_failure}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_succ.png}
  \subcaption{}
  \label{fig:obs_succ}
\end{subfigure}%
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/obs_avoidance_1_10_fail.png}
%   2-16
  \subcaption{}
  \label{fig:obs_fail}
\end{subfigure}%
\caption{Comparison of NCBFs that pass and fail the proposed verification. We shows $-0.05$, $0$, and $0.05$ level set boundaries in blue, black, and yellow lines, respectively, initial region in green and the unsafe region in red. (a) and (b) visualize NCBFs for Darboux. (c) and (d) shows projection of NCBFs for Obstacle Avoidance. }
\label{fig:DarbouxRes}
\end{figure}
\subsection{Experiment Results}
We first verify that $\mathcal{D} \subseteq \mathcal{C}$ in the Darboux and obstacle avoidance scenarios. 
We trained four $1$ hidden layer NCBFs with  $20$, $5$, $20$, $10$ neurons, respectively. 
NCBF (a) and (c) completed training, (b) terminated after $3$ epochs and (d) terminated after $5$ epochs. Our verification algorithm identifies safety violations. NCBF (a) and (c) pass the verification while NCBF (b) and (d) fail. As shown in Fig. \ref{fig:Darboux_succ}, the fully-trained NCBF (a) separates the safe and unsafe regions while the NCBF (b) with unfinished training has a boundary that intersects the unsafe region in Fig. \ref{fig:Darboux_failure}. 
As shown in Fig. \ref{fig:obs_fail}, the 2-D projection with $\psi=-1.5$ of NCBF (d) shows its boundary overlap the unsafe region. 

We next verify the positive invariance of $\mathcal{D}$. All NCBFs for Darboux pass feasibility verification with run-time presented in Table \ref{tab:NBFcomparison}. We compare the run-time of proposed verification with SMT-based approaches using translator proposed in~\cite{abate2021fossil} and SMT solver dReal~\cite{gao2013dreal} and Z3~\cite{de2008z3}. 
We can find the proposed method can verify NCBFs with more ReLU neurons while SMT-based approaches return nothing within $1$ hour time limit. 
% \textcolor{blue}{discuss improvement}
% One of the reason of improvement in performance is that we can reduce complexity by only considering the exact safety boundaries, while SMT-based approaches need to search over a safety critical subset of the state space.  
\begin{table}[!htbp]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Models & n & NN Strucutre  & $t_e$ & $t_v$  & $T$ & $T_{dReal}$ & $T_{Z3}$ \\ \hline
 & 2 & 2-20-$\sigma$-1         & 0.39 & 0.04 & 0.43    & 0.36 & Null \\
 & 2 & 2-32-$\sigma$-1         & 0.23 & 0.03 & 0.27    & 1.27 & Null \\
Darboux & 2 & 2-64-$\sigma$-1         & 1.89 & 0.13 & 2.02    & Null & Null \\
 & 2 & 2-96-$\sigma$-1         & 4.17 & 0.14 & 4.31    & Null & Null \\
 & 2 & 2-128-$\sigma$-1         & 4.77 & 0.03 & 4.90    & Null & Null \\ \hline
 & 2 & 2-10-$\sigma$-10-$\sigma$-1 & 0.42 & 0.05 & 0.47    & 7.70 & 15.81   \\ 
 & 2 & 2-16-$\sigma$-16-$\sigma$-1 & 2.13 & 0.11 & 2.23    & Null & Null   \\ 
Darboux & 2 & 2-32-$\sigma$-32-$\sigma$-1 & 8.35 & 6.28 & 14.64    & Null & Null   \\ 
 & 2 & 2-48-$\sigma$-48-$\sigma$-1 & 13.69 & 0.19 & 13.88    & Null & Null   \\ 
 & 2 & 2-64-$\sigma$-64-$\sigma$-1 & 31.30 & 0.47 & 31.77  & Null & Null   \\ \hline
\end{tabular}
\caption{Comparison of verification run-time of NCBF in seconds. We list number of dimension as $n$, network architecture with $\sigma$ denoting ReLU and run-time of proposed method including time of enumerating, verification and total run-time as $t_e$,$t_v$ and $T$, respectively. We compare with the run-time of dReal and Z3 denoted as $T_{dReal}$ and $T_{Z3}$, respectively. We write $Null$ when the program does not terminate in an hour}
\label{tab:NBFcomparison}
\end{table}

We have all NCBFs for obstacle avoidance and spacecraft rendezvous pass the verification. The run-time are presented in Table \ref{tab:NCBFcomparison}. 
We can find that the activation sets size grow steadily with the size of neural network increasing, and the number of dimension has the commanding influence on the size. The run-time is determined by both state dimension and number of ReLU hidden layers. Methods deriving tighter bounds than IBP may mitigate the influence of the ReLU hidden layers. 
% We further visualize the trend of the number of activation sets and run-time with respect to the total number of neurons with ReLU activation function in Fig. \ref{fig:trend} in supplementary material. We can find that the logarithm activation sets size grow steadily with the size of neural network increasing, while the number of dimension has the commanding influence on the size. The logarithm run-time determined by both state dimension and number of ReLU hidden layers. The potential result can be cause by loose activation set estimation. Methods deriving tighter bounds than IBP may mitigate the influence of the ReLU hidden layers. 

% The proposed exact verification do not depend on the quality of nominal controller while existing works are sufficient verification and rely on nominal controllers to conduct neural barrier certificate. 
We next show that nominal controllers can create false negative counter examples resulting a valid NCBF failing the verification. The NCBF for obstacle avoidance with one hidden layer and $32$ neurons fails the SMT-based verification using dReal given nominal controller $u$. The counter example we have is around the point $(-0.20, 0, -0.73)$. At this point, we have $b(x)=0.0033$, $\frac{\partial b}{\partial x}f(x)=0.0095$, which should be safe using sufficient condition verification. However, the nominal controller makes $\frac{\partial b}{\partial x}(f(x)+g(x)u)=-1.30$ and results in failure of verification. 

\begin{table}[!htbp]
\centering
\begin{tabular}{c|c|c|c|c|c}
\hline
Models  & n & NN Strucutre        & $t_e$ & $t_v$  & $T$ \\ \hline
 & 3 & 3-32-$\sigma$-1         & 6.94 & 0.40 & 7.35  \\
Obstacle  & 3 & 3-64-$\sigma$-1         & 19.17 & 1.87 & 21.05  \\
Avoidance  & 3 & 3-96-$\sigma$-1         & 58.96 & 6.26 & 65.22  \\
  & 3 & 3-128-$\sigma$-1         & 169.51 & 15.56 & 185.07  \\ 
\hline
  & 3 & 3-16-$\sigma$-16-$\sigma$-1 & 18.72 & 2.66 & 21.39 \\ 
Obstacle  & 3 & 3-32-$\sigma$-32-$\sigma$-1 & 218.86 & 54.51 & 273.37 \\
Avoidance  & 3 & 3-48-$\sigma$-48-$\sigma$-1 & 3197.59 & 9.75 & 3207.34 \\ 
  & 3 & 3-64-$\sigma$-64-$\sigma$-1 & 11730.28 & 18.22 & 11748.50 \\\hline
Spacecraft  & 6 & 6-8-$\sigma$-8-$\sigma$-8-1 & 78.77 & 10.23  & 89.00  \\ 
Rendezvous  & 6 & 6-16-$\sigma$-16-$\sigma$-16-1 & 1261.60 & 501.06 & 1762.67  \\ 
 & 6 & 6-32-$\sigma$-32-$\sigma$-32-1 & 12108.11 & 1798.08 & 13906.19  \\ \hline
\end{tabular}
\caption{Comparison of verification run-time of NCBF in seconds. }
\label{tab:NCBFcomparison}
\end{table}



% 32 counter-example 
% 0.099999237060546878, -1.8141281127929685, 0.51555564880371096
% dbdxf = -1.1600 dbdxg = 0.6226
% Counterexample Found: x0 : [-0.19999999825377018, -0.19999847260187381]
% x1 : [2.6428997918226282e-05, 2.9071897710048909e-05]
% x2 : [-0.72578002929687502, -0.7257785320281982]
% -(bv+u)
% Out[15]: tensor(-1.3062)
% bv
% Out[16]: tensor(-0.0951)
% u
% Out[17]: tensor(1.4013)


==> backup/Experiment_SupplementV1.tex <==
\subsection{Darboux}
\label{sup:darboux}
We first show verification of a neural barrier function for Darboux system whose dynamic is defined as follow. 
\begin{equation}
    \left[\begin{array}{c}
    \dot{x}_1 \\
    \dot{x}_2
    \end{array}\right]=\left[\begin{array}{c}
    x_2+2 x_1 x_2 \\
    -x_1+2 x_1^2-x_2^2
    \end{array}\right].
\end{equation}
We define state space, initial region, and unsafe region as $\mathcal{X}:\left\{\mathbf{x} \in \mathbb{R}^2: x\in[-2,2]\times[-2,2] \right\}$, $\mathcal{X}_I:\left\{\mathbf{x} \in \mathbb{R}^2: 0 \leq x_1 \leq 1,1 \leq x_2 \leq 2\right\}$ and $\mathbf{x}_{U}:\left\{\mathbf{x} \in \mathbb{R}^2: x_1+x_2^2 \leq 0\right\}$ respectively. 

\subsection{Obstacle Avoidance}
\label{sup:obstacle}
We next evaluate that our proposed method on a controlled system~\cite{barry2012safety}. The system state  consists of 2-D position and aircraft yaw rate $x:=[x_1, x_2, \psi]^T$. We let $u$ denote the control input to manipulate yaw rate and define the dynamics as
\begin{equation}
    \left[\begin{array}{c}
    \dot{x}_1 \\
    \dot{x}_2 \\
    \dot{\psi}
    \end{array}\right]=\left[\begin{array}{c}
    v \sin \psi \\
    v \cos \psi \\
    0
\end{array}\right]
+ \left[\begin{array}{c}
    0 \\
    0 \\
    u
\end{array}\right]. 
\end{equation}
We define the state space, initial region and unsafe region as $\mathcal{X}$, $\mathcal{X}_I$ and $\mathcal{X}_U$, respectively as 
\begin{equation}
    \begin{aligned}
    \mathcal{X}:&\left\{\mathbf{x} \in \mathbb{R}^3:x_1,x_2,\psi\in [-2,2]\times[-2,2]\times[-2,2] \right\} \\
    \mathcal{X}_I:&\left\{\mathbf{x} \in \mathbb{R}^3:-0.1 \leq x_1 \leq 0.1,-2 \leq x_2 \leq-1.8, \ -\pi/6<\psi<\pi / 6 \right\} \\
    \mathcal{X}_U:&\left\{\mathbf{x} \in \mathbb{R}^3: x_1^2+x_2^2 \leq 0.04\right\}
\end{aligned}
\end{equation}

\subsection{Spacecraft Rendezvous}
\label{sup:Spacecraft}
The state of the chaser is expressed relative to the target using linearized Clohessy–Wiltshire–Hill equations, with state $x=[p_x, p_y, p_z, v_x, v_y, v_z]^T$, control input $u=[u_x, u_y, u_z]^T$ and dynamics defined as follows. 
\begin{equation}
    \left[\begin{array}{c}
    \dot{p}_x \\
    \dot{p}_y \\
    \dot{p}_z \\
    \dot{v}_x \\
    \dot{v}_y \\
    \dot{v}_z
    \end{array}\right]=
    \left[\begin{array}{c c c c c c}
    1 &0 &0 &0 &0 &0 \\
    0 &1 &0 &0 &0 &0 \\
    0 &0 &1 &0 &0 &0 \\
    3n^2 &0 &0 &0 &2n &0 \\
    0 &0 &0 &-2n &0 &0 \\
    0 &0 &-n^2 &0 &0 &0 
    \end{array}\right]
    \left[\begin{array}{c}
    p_x \\
    p_y \\
    p_z \\
    v_x \\
    v_y \\
    v_z
    \end{array}\right]
+ \left[\begin{array}{c c c}
    0 &0 &0 \\
    0 &0 &0 \\
    0 &0 &0 \\
    1 &0 &0 \\
    0 &1 &0 \\
    0 &0 &1
\end{array}\right]
\left[\begin{array}{c}
    u_x \\
    u_y \\
    u_z 
    \end{array}\right]. 
\end{equation}
We define the state space and unsafe region as $\mathcal{X}$ and $\mathcal{X}_U$, respectively as 
\begin{equation}
    \begin{aligned}
    \mathcal{X}:&\left\{\mathbf{x} \in \mathbb{R}^3: p, v, \in [-1.5,1.5]\times[-1.5,1.5]\right\} \\
    \mathcal{X}_U:&\left\{ 0.25 \leq r \leq 1.5\text{, where } r=\sqrt{p_x^2+ p_y^2+ p_z^2} \right\}
\end{aligned}
\end{equation}
We obtain the trained NCBF with neural CLBF training in~\cite{dawson2023safe} with a nominal model predictive controller. 
% In this experiment, we observe the increasing dimension can highly increase time consumed for gridifying the state space and LiRPA. Instead, we enumerate $2^8$ activation sets and verified the NCBF.

\subsection{Training Details}
\label{subsec:training_details}
We trained the NBFs for Darboux and NCBFs for obstacle avoidance via the approach proposed in \cite{zhao2020synthesizing}, which we summarize as follows. We first sample points from the state space, initial region, and unsafe region separately to generate data for training denoted as $D_D$, $D_I$, and $D_U$ respectively. We then trained our NBFs and NCBFs with loss function  
\begin{equation*}
    C\left(D_D, D_I, D_U\right)=\sum_{\mathbf{x} \in D_D} C_D(\mathbf{x})+\sum_{\mathbf{x} \in D_I} C_I(\mathbf{x})+\sum_{\mathbf{x} \in D_U} C_U(\mathbf{x}),
\end{equation*}
where $C_D, C_I, C_U: \mathbb{R}^{n} \rightarrow \mathbb{R}$ are sub-loss functions derived from Theorem 2.3 of  \cite{zhao2020synthesizing}. Detailed parameters for both cases are listed in Table \ref{tab:hyperpara_NBF}. 

We then trained NCBFs for Spacecraft Rendezvous by following approach proposed in \cite{dawson2023safe} with the empirical loss defined in Eq. (5) in \cite{dawson2022safe}. The hyper-parameters are listed in Table \ref{tab:hyperpara_NCBF}. 


\begin{table}[!htbp]
\begin{subtable}[]{0.45\textwidth}
\begin{tabular}{l|l}
Hyper-Parameters & Value \\ \hline
LEARNING\_RATE & 0.01  \\
LOSS\_OPT\_FLAG & 1e-16 \\
TOL\_MAX\_GRAD & 6 \\
EPOCHS & 5 \\
TOL\_INIT & 0.0  \\
TOL\_SAFE & 0.0 \\
TOL\_BOUNDARY & 0.05 \\
TOL\_LIE & 0.0 \\
TOL\_NORM\_LIE & 0.0 \\
WEIGHT\_LIE & 1 \\
WEIGHT\_NORM\_LIE & 0 \\
DECAY\_LIE & 1 \\
DECAY\_INIT & 1 \\
DECAY\_UNSAFE & 1 \\
\hline               
\end{tabular}

\subcaption[]{Hyper-parameters for Darboux and Obstacle Avoidance}
\label{tab:hyperpara_NBF}
\end{subtable}
% \hfill
\begin{subtable}[h]{0.45\textwidth}
\begin{tabular}{l|l}
Hyper-Parameters & Value \\ \hline
LEARNING\_RATE & 0.01  \\
BATCH\_SIZE & 512\\
CONTROLLER\_PERIOD & 0.01\\
SIMULATION\_DT & 0.01\\
CBF\_HIDDEN\_LAYERS&1\\
CBF\_HIDDEN\_SIZE&16\\
CBF\_LAMBDA&0.1\\
CBF\_RELAXATION\_PENALTY & 1e4\\
SCALE\_PARAMETER&10.0\\
PRIMAL\_LEARNING\_RATE & 1e-3\\
LEARN\_SHAPE\_EPOCHS&100\\
\hline
\end{tabular}
\subcaption[]{Hyper-parameters for Spacecraft Randezvous}
\label{tab:hyperpara_NCBF}
\end{subtable}
\label{tab:hyperpara}
\caption{Hyper-parameters for training NBFs and NCBFs to be verified}
\end{table}

\subsection{Experiment Details}

\subsection{Experiment Results}
We further visualize the trend of the number of activation sets and run-time with respect to the total number of neurons with ReLU activation function in Fig. \ref{fig:trend} in supplementary material. We can find that the logarithm activation sets size grow steadily with the size of neural network increasing, while the number of dimension has the commanding influence on the size. The logarithm run-time is determined by both state dimension and number of ReLU hidden layers. The potential result can be cause by loose activation set estimation. Methods deriving tighter bounds than IBP may mitigate the influence of the ReLU hidden layers. 
\begin{figure}[!htbp]
\centering
\begin{subfigure}{.45\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{figs/LogActSetCmp.png}
  \subcaption{}
  \label{fig:num_act}
\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/LogRuntimeComp.png}
%   2-16
  \subcaption{}
  \label{fig:runtime}
\end{subfigure}%
\caption{Comparison of the number of activation sets and run-time with respect to number of neurons in total. (a) shows logarithm of activation set size. (b) shows logarithm of run-time. We denote NBFs for Darboux with 1 and 2 hidden layers as Darboux 1 and Darboux 2, respectively. We denote NCBFs for obstacle avoidance with 1 and 2 hidden layers as obs 1 and obs 2, respectively.}
\label{fig:trend}
\end{figure}

==> backup/Experiment_backup.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we evaluate our proposed method to verify neural control barrier functions on three systems. We first consider the Darboux system~\cite{zeng2016darboux}, a nonlinear open-loop polynomial system that has been widely used for safety verification. We then evaluate our approach on an obstacle avoidance scenario~\cite{barry2012safety}. We finally evaluate our approach on a spacecraft rendezvous problem from~\cite{jewison2016spacecraft}. The experiments run on a 64-bit Windows PC with Intel(R) Core(TM) i7-12700 processor, 32GB RAM and NVIDIA GeForce RTX 3080 GPU. 

\subsection{Darboux}
We first show verification of a neural barrier function for Darboux system whose dynamic is defined as follow. 
\begin{equation}
    \left[\begin{array}{c}
    \dot{x}_1 \\
    \dot{x_2}
    \end{array}\right]=\left[\begin{array}{c}
    x_2+2 x_1 x_2 \\
    -x_1+2 x_1^2-x_2^2
    \end{array}\right].
\end{equation}
We define state space, initial region, and unsafe region as $\mathcal{X}:\left\{\mathbf{x} \in \mathbb{R}^2: x\in[-2,2]\times[-2,2] \right\}$, $\mathcal{X}_I:\left\{\mathbf{x} \in \mathbb{R}^2: 0 \leq x_1 \leq 1,1 \leq x_2 \leq 2\right\}$ and $\mathbf{x}_{U}:\left\{\mathbf{x} \in \mathbb{R}^2: x_1+x_2^2 \leq 0\right\}$ respectively. 

We first show an example of correctness verification. We construct a neural barrier function with one hidden layer consisting of 20 neurons followed with a ReLU activation function. We  trained two NBFs that (a) terminated after $3$ epochs and (b) completed training. As shown in Fig. \ref{fig:Darboux_failure}, the NBF with unfinished training has a boundary that intersects the unsafe region, hence, this barrier function is used to test whether our approach can correctly identify that an NBF does not ensure safety. The fully-trained NBF  has a boundary shown in Fig. \ref{fig:Darboux_succ} that  separates the safe and unsafe regions. 

We next verify the NBFs with our proposed method and compared our total run time with state-of-the-art SMT-based verification, dReal and Z3. We first verified a network with 1 ReLU hidden layer and 20 neurons in each hidden layer. The NBF passed all components of the verification after $0.43s$ seconds(s) in total. The enumerating procedure takes $0.39s$ to find $13$ activation set and intersections. The sufficient condition verification takes $0.04s$. The SMT-based verification dReal verified the NBF in $0.36s$ in total. The SMT-based verification Microsoft Z3 cannot finish within an hour when verifying the NBF. 
We first verified a network with 2 ReLU hidden layer and 10 neurons in each hidden layer. The NBF passed all components of the verification after $0.47s$ seconds(s) in total. The enumerate set procedure takes $0.42s$ to find $4$ activation set and intersections. The sufficient condition verification takes $0.05s$. The SMT-based verification takes $7.70s$ with dReal and $15.81$ with Microsoft Z3. 

\begin{figure}[!htbp]
\centering
\begin{subfigure}{.35\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{figs/darbox_1_20_failure.eps}
  \subcaption{}
  \label{fig:Darboux_failure}
\end{subfigure}%
% \hfill
\begin{subfigure}{.35\textwidth}
  \centering
  \includegraphics[width= \textwidth]{figs/darboux_1_20_lr01.eps}
%   \caption{Joint FDI and Spoofing Attack: INS2 estimation}
  \subcaption{}
  \label{fig:Darboux_succ}
\end{subfigure}%
\caption{Visualization of neural barrier functions. (a) Barrier function training with insufficient data results in a boundary (black, blue, and yellow lines) that intersects with the unsafe region (red area). Our verification algorithm identifies this safety violation. (b) Training with sufficient data results in a boundary that avoids the unsafe region.}
\label{fig:DarbouxRes}
\end{figure}

\subsection{Obstacle Avoidance}
We next evaluate that our proposed method on a controlled system~\cite{barry2012safety}. We consider an Unmanned aerial vehicle (UAVs) flying  through a forest avoiding collision with tree trunks. We model the system as a  Dubins-style \cite{dubins1957curves} aircraft model. The system state  consists of 2-D position and aircraft yaw rate $x:=[x_1, x_2, \psi]^T$. We let $u$ denote the control input to manipulate yaw rate and define the dynamics as
\begin{equation}
    \left[\begin{array}{c}
    \dot{x}_1 \\
    \dot{x}_2 \\
    \dot{\psi}
    \end{array}\right]=\left[\begin{array}{c}
    v \sin \psi \\
    v \cos \psi \\
    0
\end{array}\right]
+ \left[\begin{array}{c}
    0 \\
    0 \\
    u
\end{array}\right]. 
\end{equation}
We define the state space, initial region and unsafe region as $\mathcal{X}$, $\mathcal{X}_I$ and $\mathcal{X}_U$, respectively as 
\begin{equation}
    \begin{aligned}
    \mathcal{X}:&\left\{\mathbf{x} \in \mathbb{R}^3:x_1,x_2,\psi\in [-2,2]\times[-2,2]\times[-2,2] \right\} \\
    \mathcal{X}_I:&\left\{\mathbf{x} \in \mathbb{R}^3:-0.1 \leq x_1 \leq 0.1,-2 \leq x_2 \leq-1.8, \ -\pi/6<\psi<\pi / 6 \right\} \\
    \mathcal{X}_U:&\left\{\mathbf{x} \in \mathbb{R}^3: x_1^2+x_2^2 \leq 0.04\right\}
\end{aligned}
\end{equation}
We obtain the trained NCBF by CEGIS framework in \cite{zhao2020synthesizing} with $v$ assumed to be $1$ and the control law $u$ designed as
$ u=-\sin \psi+3 \cdot \frac{x_1 \cdot \sin \psi+x_2 \cdot \cos \psi}{0.5+x_1^2+x_2^2}$. 

We next verify the NCBFs with our proposed method. We first verified a network with 1 ReLU hidden layer and 50 neurons in each hidden layer. The NCBF passed all components of the verification after $13.86s$ in total. The enumerating procedure takes $12.81s$ to find $966$ activation set and intersections. The sufficient condition verification takes $1.06s$. 
We then verified a network with 2 ReLU hidden layer and 32 neurons in each hidden layer. The NBF passed all components of the verification after $273.37s$ seconds(s) in total. The enumerate set procedure takes $218.86s$ to find $1317$ activation set and intersections. The sufficient condition verification takes $54.51s$. 

\subsection{Spacecraft Rendezvous}
The state of the chaser is expressed relative to the target using linearized Clohessy–Wiltshire–Hill equations, with state $x=[p_x, p_y, p_z, v_x, v_y, v_z]^T$, control input $u=[u_x, u_y, u_z]^T$ and dynamics defined as follows. 
\begin{equation}
    \left[\begin{array}{c}
    \dot{p}_x \\
    \dot{p}_y \\
    \dot{p}_z \\
    \dot{v}_x \\
    \dot{v}_y \\
    \dot{v}_z
    \end{array}\right]=
    \left[\begin{array}{c c c c c c}
    1 &0 &0 &0 &0 &0 \\
    0 &1 &0 &0 &0 &0 \\
    0 &0 &1 &0 &0 &0 \\
    3n^2 &0 &0 &0 &2n &0 \\
    0 &0 &0 &-2n &0 &0 \\
    0 &0 &-n^2 &0 &0 &0 
    \end{array}\right]
    \left[\begin{array}{c}
    p_x \\
    p_y \\
    p_z \\
    v_x \\
    v_y \\
    v_z
    \end{array}\right]
+ \left[\begin{array}{c c c}
    0 &0 &0 \\
    0 &0 &0 \\
    0 &0 &0 \\
    1 &0 &0 \\
    0 &1 &0 \\
    0 &0 &1
\end{array}\right]
\left[\begin{array}{c}
    u_x \\
    u_y \\
    u_z 
    \end{array}\right]. 
\end{equation}
We define the state space, initial region and unsafe region as $\mathcal{X}$, $\mathcal{X}_I$ and $\mathcal{X}_U$, respectively as 
\begin{equation}
    \begin{aligned}
    \mathcal{X}:&\left\{\mathbf{x} \in \mathbb{R}^3: p, v, \in [-1.5,1.5]\times[-1.5,1.5]\right\} \\
    \mathcal{X}_U:&\left\{ 0.25 \leq r \leq 1.5\text{, where } r=\sqrt{p_x^2+ p_y^2+ p_z^2} \right\}
\end{aligned}
\end{equation}

We obtain the trained NCBF with neural CLBF training in~\cite{dawson2023safe} with a nominal model predictive controller. We next verify the NCBFs with our proposed method. We first verified a NCBF who has 2 ReLU hidden layers with 8 neurons in each hidden layer and 1 hidden layer with linear activation function. The NCBF passed all components of the verification after $47.45s$ in total. The enumerating procedure takes $47.45s$ to find $273$ activation set and intersections. The sufficient condition verification takes $0.08s$. In this experiment, we observe the increasing dimension can highly increase time consumed for gridifying the state space and LiRPA. Instead, we enumerate $2^8$ activation sets and verified the NCBF. 

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Models  & Type & n & NN Strucutre        & $t_e$ & $t_v$  & $T$ & $T_{dReal}$ & $T_{Z3}$ \\ \hline
Darboux & NBF  & 2 & 2-20-$\sigma$-1         & 0.39 & 0.04 & 0.43    & 0.36 & Null \\
Darboux & NBF  & 2 & 2-32-$\sigma$-1         & 0.23 & 0.03 & 0.27    & 1.27 & Null \\
Darboux & NBF  & 2 & 2-64-$\sigma$-1         & 1.89 & 0.13 & 2.02    & Null & Null \\
Darboux & NBF  & 2 & 2-96-$\sigma$-1         & 4.17 & 0.14 & 4.31    & Null & Null \\
Darboux & NBF  & 2 & 2-128-$\sigma$-1         & 4.77 & 0.03 & 4.90    & Null & Null \\ \hline
Darboux & NBF  & 2 & 2-10-$\sigma$-10-$\sigma$-1 & 0.42 & 0.05 & 0.47    & 7.70 & 15.81   \\ 
Darboux & NBF  & 2 & 2-16-$\sigma$-16-$\sigma$-1 & 2.13 & 0.11 & 2.23    & Null & Null   \\ 
Darboux & NBF  & 2 & 2-32-$\sigma$-32-$\sigma$-1 & 8.35 & 6.28 & 14.64    & Null & Null   \\ 
Darboux & NBF  & 2 & 2-48-$\sigma$-48-$\sigma$-1 & 13.69 & 0.19 & 13.88    & Null & Null   \\ 
Darboux & NBF  & 2 & 2-64-$\sigma$-64-$\sigma$-1 & 31.30 & 0.47 & 31.77  & Null & Null   \\ \hline
Obstacle & NCBF & 3 & 3-32-$\sigma$-1         & 6.94 & 0.40 & 7.35  & Fail  & Fail \\
Obstacle & NCBF & 3 & 3-64-$\sigma$-1         & 19.17 & 1.87 & 21.05  & Null  & Null \\
Obstacle & NCBF & 3 & 3-96-$\sigma$-1         & 58.96 & 6.26 & 65.22  & Null  & Null \\
Obstacle & NCBF & 3 & 3-128-$\sigma$-1         & 169.51 & 15.56 & 185.07  & Null  & Null \\ 
\hline
Obstacle & NCBF & 3 & 3-16-$\sigma$-16-$\sigma$-1 & 18.72 & 2.66 & 21.39 & Fail & Fail \\ 
Obstacle & NCBF & 3 & 3-32-$\sigma$-32-$\sigma$-1 & 218.86 & 54.51 & 273.37 & Null & Null \\
Obstacle & NCBF & 3 & 3-48-$\sigma$-48-$\sigma$-1 & 3197.59 & 9.75 & 3207.34 & Null & Null \\ 
Obstacle & NCBF & 3 & 3-64-$\sigma$-64-$\sigma$-1 & 11730.28 & 18.22 & 11748.50 & Null & Null \\\hline
\begin{tabular}[c]{@{}c@{}}Spacecraft \\ Rendezvous\end{tabular} & NCBF & 6 & 6-8-$\sigma$-8-$\sigma$-8-1 & 47.37  & 0.08  & 47.45  & None & None \\ \hline
\end{tabular}
\caption{Comparison of verification mean run-time of NBF and NCBF in seconds over 10 trails. We list number of dimension as $n$, network architecture with $\sigma$ denoting ReLU and run-time of proposed method including time of enumerating $t_e$, time of verification $t_v$ and time in total $T$. We compare the run-time proposed verification of NBF with SMT-based approaches, i.e., dReal $T_{dReal}$ and Z3 $T_{Z3}$.  }
\label{tab:comparison}
\end{table}

% 16-16 counter-example
% -0.18750， 0.013552790， -0.71100797
% dbdxf = tensor(-0.6340) dbdxg = 0.1366

% 32 counter-example 
% 0.099999237060546878, -1.8141281127929685, 0.51555564880371096
% dbdxf = -1.1600 dbdxg = 0.6226

==> backup/IntroV1.tex <==
\section{Introduction}
Safety is a critical property for autonomous systems, including unmanned ground, aerial, and space vehicles \cite{agrawal2021safe} and robotic manipulators \cite{hsu2015control}. The importance of safety has motivated extensive research into verification and synthesis of safe control strategies for autonomous systems \cite{xu2017correctness}. Control barrier function (CBF)-based algorithms \cite{ames2019control} ensure safety by  constructing a CBF that is nonnegative if the system is safe (a property we denote as \emph{correctness}) and synthesizing a control policy that ensures that the CBF is nonnegative for all time (a property we denote as \emph{feasibility}). Control barrier functions provide a high degree of flexibility, since any control policy that satisfies the control barrier function constraint is provably safe, and have been demonstrated in applications including \cite{ames2014control,chen2020guaranteed,xu2017correctness}. Recently, CBFs that are parametrized by neural networks (\emph{neural control barrier functions} or  NCBFs~\cite{dawson2022safe,dawson2023safe,liu2023safe}) have been proposed. While this novel class of NCBFs is promising due to the universal representability of neural networks (enabling the encoding of complex safety constraints) as well as the efficiency of learning algorithms, verification of NCBFs remains a challenging research problem.  

%To describe complex safety constraints, \emph{neural control barrier functions} (NCBFs)~\cite{dawson2022safe,dawson2023safe,liu2023safe} have been proposed to exploit the universal representability as well as the efficiency of learning algorithms. 

%In particular, energy-based methodologies such as barrier certificates \cite{prajna2007framework} and control barrier functions \cite{ames2019control} have been proposed that construct an energy function that is positive if the system is safe, and then guarantee safety by proving that the barrier function remains positive for all time. These methods generalize classic Lyapunov-methods for proving stability \cite{ames2014control}. Control barrier functions provide a high degree of flexibility, since any control policy that satisfies the control barrier function constraint is provably safe. To describe complex safety constraints, \emph{neural control barrier functions} (NCBFs)~\cite{dawson2022safe,dawson2023safe,liu2023safe} have been proposed to exploit the universal representability as well as the efficiency of learning algorithms. 

%CBFs and NCBFs, however, may fail to guarantee safety for two reasons, namely, correctness and feasibility. Correctness requires NCBFs to not overlap with unsafe region. Feasibility requires that there always exist a control input that satisfies NCBF conditions. Furthermore, an example in Section \ref{subsec:safety-conditions} shows some points can cause safety violations. The safety properties of NCBF-based systems must be verified in order to have a provable safety guarantee in safety-critical autonomous CPS. Neural barrier certificate was proposed in \cite{zhao2020synthesizing, abate2021fossil} to find safety counterexamples by verifying the close-loop system with a given or synthesized nominal controller. However, these methods are dependent on the quality of nominal controllers. Specifically, a valid NCBF may still fail the verification if the given or synthesized controller fail to find a feasible control input. 

In this paper, we consider the problem of verifying safety of a nonlinear continuous-time system using an NCBF represented by a feed-forward neural network with ReLU activation function. We choose the ReLU function because of its widespread use in NN learning including for NCBFs \cite{dawson2022safe,dawson2023safe}. The key challenge for this class of NCBFs is that most methodologies for safety verification are based on proving that the derivative of the barrier function is nonnegative at the boundary of the safe region, and hence the barrier function remains nonnegative for all time. Since the ReLU activation function is not continuously differentiable, this approach is inapplicable. We resolve this challenge and derive exact safety conditions for ReLU NCBFs  by leveraging a generalization of Nagumo's theorem for proving invariance of sets with nonsmooth boundaries. Our safety conditions also incorporate linear constraints on the control input, which may arise due to limits on actuation.

We  propose an algorithm to verify these safety conditions. Our approach first decomposes the NCBF into piecewise linear segments. In order to mitigate the complexity of this stage, we show that it suffices to consider linear segments at the boundary of the safe region, and further over-approximate the segments using Interval Bound Propagation and linear relaxation. After decomposing the NCBF, we then verify safety by solving a set of nonlinear programs, which satisfy the safety criteria on each linear segment as well as at intersections of the segments. The nonlinearity arises due to the nonlinearity of the system dynamics. We evaluate our approach through numerical studies, in which we verify NBFs and NCBFs with our proposed approach and compare to state-of-the-art SMT-based methods. 



%We propose an algorithm for safety verification that first decomposes the NCBF into piecewise linear segments and then solves a nonlinear program to verify safety of each segment as well as the intersections of the linear segments. We further mitigate the complexity by only considering the boundary of the safe region and prune the segments with Interval Bound Propagation (IBP) and linear relaxation. In particular, we made the following core contributions.  

% \item We prove that safety verification of an NCBF is equivalent to verifying safety at a subset of the boundary of the safe region. We characterize this boundary as the union of a collection of inputs that activate different subsets of neurons, and propose an algorithm for constructing the safety boundary by enumerating all such activation sets.
%We formulate a novel necessary and sufficient condition for positive invariance of the level set of a neural network. This condition generalizes the safety conditions of control barrier functions to neural control barrier functions where the gradient of the neural network is not well-defined. 

%We propose a novel framework to analyze ReLU NCBFs. The framework can be summarized as coarser-to-finer search for safety critical subsets and verification of subsets. We gridify the state space, over-estimate possible critical sets and identify the critical sets using linear programing. We formulate the problem of ensuring that, for each verification region, there is no system state that leads to safety violation. 
% \item We formulate the problem of ensuring that, for each verification region, there is no system state that leads to safety violation. We map this problem to a nonlinear program and incorporate constraints on actuation. 



\textbf{Related Work}
Energy-based methods are proposed to guarantee safety by ensuring that a particular energy function remains nonnegative. Barrier certificates for safe control were first proposed in \cite{prajna2007framework} to verify safety of a given system. More recently, CBFs have recently emerged as promising approaches to safe control, due to their compatibility with a wide variety of control laws \cite{ames2019control}. CBFs have been led to theoretical exploration of safe control under high-order dynamics \cite{xiao2019control, clark2021verification}, actuation constraints \cite{dai2022convex, liu2023safe, dawson2022safe,agrawal2021safe}, and other properties. 

Sum-of-squares optimization and other techniques derived from algebraic geometry have been widely used for safety verification of polynomial barrier functions \cite{prajna2007framework,ames2019control,zhao2022safety}. An algebraic-geometric method is proposed in~\cite{schneeberger2023sos,clark2021verification} to verify CBFs using sum-of-squares (SOS) optimization programs derived from the Positivstellensatz \cite{parrilo2003semidefinite}. However, traditional SOS-based approach cannot be directly applied for NBF/NCBF verification, since activation functions used in neural networks are not polynomial and can be non-differentiable. 

Emerging approaches, NBFs~\cite{berkenkamp2017safe,abate2021fossil,qin2021learning} and NCBFs~\cite{dawson2022safe,dawson2023safe,liu2023safe} are proposed to describe complex safety constraints that cannot be encoded polynomials. Neural barrier certificates learn a barrier function that describes the safety of a given dynamical system \cite{zhao2020synthesizing, abate2021fossil}, while neural control barrier functions jointly learn a control policy and a barrier function that certifies safety of that policy \cite{dawson2022safe}. In both cases, the barrier function is typically learned by constructing a loss function that encodes the safety constraints of the system \cite{boffi2021learning}. Since the barrier function is computed from training data which are inherently incomplete, the neural barrier function must be verified to ensure that it correctly enforces the safety constraint. 
Current work focus on verifying NBFs including SMT-based method \cite{zhao2020synthesizing,abate2021fossil} and nonlinear mixed integer programs \cite{zhao2022verifying} and leave exact verification for NCBFs less studied. 

Another related body of work deals with the problem of verifying neural networks, e.g., determining whether a neural network output is nonnegative for any input within a particular range. Neural network verification include Satisfiability Modulo Theory \cite{scheibler2013recent}, output reachable set verification \cite{xiang2018output} and polynomial approximations of the barrier function~\cite{sha2021synthesizing}. Significant recent advances, especially in verification of ReLU neural networks, have led to methodologies that scale to neural networks with hundreds or even thousands of neurons \cite{katz2017reluplex,katz2019marabou}. These methods, however, are not directly applicable to the problem of NCBF verification, because it requires joint consideration of the neural network and the underlying nonlinear system dynamics. 

\textbf{Organization} The remainder of the paper is organized as follows. Section \ref{sec:preliminaries} gives the system model and background on neural networks and notation. Section \ref{sec:safety_conditions} presents the problem formulation and exact conditions for safety. Section \ref{sec:verification} presents our approach to verifying each sub-region of the safety boundary and gives the overall safety proof of our approach. Section \ref{sec:experiments} contains simulation results. Section \ref{sec:conclusions} concludes the paper. 

==> sections/backup_introv1.tex <==
\section{Introduction}
Safety is a critical property of control systems including unmanned ground, aerial, and space vehicles \textbf{*ref} and robotic manipulators \textbf{*ref}. From a control-theoretic perspective, safety can be modeled as ensuring that the system state avoids an unsafe set, for example, avoiding obstacles or maintaining velocity or attitude within a desired tolerance region. 

The importance of safety has motivated extensive research into verification and synthesis of safe control strategies for autonomous systems \cite{xu2017correctness}. In particular, energy-based methodologies such as barrier certificates \cite{prajna2007framework} and control barrier functions \cite{ames2019control} have been proposed that construct an energy function that is positive if the system is safe, and then prove safety by proving that the system remains positive for all time. These methods generalize classic Lyapunov-methods for proving stability \cite{ames2014control}. Control barrier functions provide a high degree of flexibility, since any control policy that satisfies the control barrier function constraint is provably safe. More recently, \emph{neural control barrier functions} (NCBFs)~\cite{dawson2022safe,dawson2023safe,liu2023safe} have been proposed to exploit the universal representability as well as the efficiency of NN learning algorithms to describe complex safety constraints that cannot be encoded polynomials. Neural control barrier functions jointly learn a control policy and a barrier function that certifies safety of that policy. While most existing works focus on learning barrier certificates. 
% \emph{neural barrier functions} (NBFs)~\cite{berkenkamp2017safe,abate2021fossil,qin2021learning} 

A CBF may fail to guarantee safety for two reasons. First, the NCBF may overlap with unsafe region, referred to as correctness. Second, there may not exist control input that satisfy NCBF conditions, referred to as feasibility. Furthermore, Example in Section \ref{subsec:safety-conditions} shows some points can case safety violations. In order to ensure trust and confidence in safety-critical autonomous CPS, the safety properties of NCBF-based systems must be verified. Neural barrier certificate was proposed in \cite{zhao2020synthesizing, abate2021fossil} to ensure safety by finding counterexamples. However, these methods rely on nominal controllers for neural barrier certificate and cannot verify NCBF. 

In this paper, we consider the problem of verifying safety of a nonlinear control system using a NBF represented by a feedforward neural network with ReLU activation function. We choose the ReLU function because of its widespread use in NN learning including for NCBFs. We reduce the complexity of the verification by exploiting two key features of the verification problem. First, it is sufficient to verify safety at a subset of critical states that lie at the boundary between the safe and unsafe regions. We propose an algorithm for characterizing the set of such critical states. Second, we derived exact conditions for NCBF verification. A ReLU-based NCBF is piece-wise linear, which enables us to decompose the verification problem into a collection of nonlinear programs. In particular, we made the following contributions: 
\begin{itemize}
\item We prove that safety verification of an NCBF is equivalent to verifying safety at a subset of the boundary of the safe region. We characterize this boundary as the union of a collection of inputs that activate different subsets of neurons, and propose an algorithm for constructing the safety boundary by enumerating all such activation sets.
\item We formulate a novel necessary and sufficient condition for positive invariance of the level set of a neural network. This condition generalizes the safety conditions of control barrier functions to barrier functions where the gradient of the barrier function is not well-defined. 
\item We formulate the problem of ensuring that, for each verification region, there is no system state that leads to safety violation. We map this problem to a nonlinear program and incorporate constraints on actuation. 
\item We evaluate our approach through numerical studies. We verify NBF and NCBFs with our proposed approach and compare to state-of-the-art SMT-based methods. 
\end{itemize}

The remainder of the paper is organized as follows. Section \ref{sec:preliminaries} gives the system model and background on neural networks and notation. Section \ref{sec:safety_conditions} presents the problem formulation and exact conditions for safety. Section \ref{sec:verification} presents our approach to verifying each sub-region of the safety boundary and gives the overall safety proof of our approach. Section \ref{sec:experiments} contains simulation results. Section \ref{sec:conclusions} concludes the paper. 

\section{Related Work}
Neural network verification include Satisfiability Modulo Theory \cite{scheibler2013recent}, output reachable set verification \cite{xiang2018output} and polynomial approximations of the barrier function~\cite{sha2021synthesizing}. These methods, however, are not directly applicable to the problem of NCBF verification, because it requires joint consideration of the neural network and the underlying nonlinear system dynamics. 
